Demonstration Attack against In-Context Learning for Code Intelligence

Recent advancements in large language models (LLMs) have revolutionized code intelligence by improving programming productivity and alleviating challenges faced by software developers. To further improve the performance of LLMs on specific code intelligence tasks and reduce training costs, researchers reveal a new capability of LLMs: in-context learning (ICL). ICL allows LLMs to learn from a few demonstrations within a specific context, achieving impressive results without parameter updating. However, the rise of ICL introduces new security vulnerabilities in the code intelligence field. In this paper, we explore a novel security scenario based on the ICL paradigm, where attackers act as third-party ICL agencies and provide users with bad ICL content to mislead LLMs outputs in code intelligence tasks. Our study demonstrates the feasibility and risks of such a scenario, revealing how attackers can leverage malicious demonstrations to construct bad ICL content and induce LLMs to produce incorrect outputs, posing significant threats to system security. We propose a novel method to construct bad ICL content called DICE, which is composed of two stages: Demonstration Selection and Bad ICL Construction, constructing targeted bad ICL content based on the user query and transferable across different query inputs. Ultimately, our findings emphasize the critical importance of securing ICL mechanisms to protect code intelligence systems from adversarial manipulation.

==> FSE25/algorithms/greedy_iterator.tex <==
\begin{algorithm}
\small
\caption{Greedy Mutation Workflow}
\label{alg:greedy_iterator}
\begin{algorithmic}[1]
    % \Statex \textbf{Input:} $demos$: ICL demonstration code, $M$: code LLM, $vars$: variables of the demonstration, $subs$: substitutes of the variable
    % \Statex \textbf{Output:} $demos'$: mutation of demonstration code
    % % \State $demos' = \emptyset$
    % \State $demo = \emptyset;$
    % % \State $vars = extract($demo$)$
    % \For{$demo$ in $demos$}
    %     \State $demo' = \emptyset;$
    %     \State $var = \emptyset;$
    %     \State $vars = \text{vul\_score}(vars));$
    %     \For{$var$ in $vars[demo]$}
    %         \State $candidate\_demo = \emptyset;$
    %         \State $sub = \emptyset;$
    %         \For{$sub$ in $subs[var]$}
    %             \State $temp\_demo = mutate(demos', var, sub);$
    %             \If{$compare(M(temp\_demo), M(demo)) = \text{true}$}
    %                 \State $demo' = temp\_demo;$
    %                 \State $demos'[demo] = demo';$
    %                 \State $\text{break};$
    %             \EndIf
    %             \State $candidate\_demo = candidate\_demo \cup temp\_demo;$
    %         \EndFor
    %         \State $demo' = select(candidate\_demo);$
    %     \EndFor
    % \EndFor
    % \State \Return $demos'$ 
    
% \State \textbf{Input:} $demos$: ICL demonstration code, $M$: code LLM, $vars$: variables of the demonstration, $subs$: substitutes of the variable
% \State \textbf{Output:} $demos'$: mutation of demonstration code
% \State $demos' \gets \emptyset$
% \For{each $demo$ in $demos$}
%     \State $demo' \gets \emptyset$
%     \State $vars \gets \text{vul\_score}(vars)$
%     \State $found \gets \text{false}$
%     \For{each $var$ in $vars[demo]$}
%         \State $candidate\_demo \gets \emptyset$
%         \For{each $sub$ in $subs[var]$}
%             \State $temp\_demo \gets \text{mutate}(demos', var, sub)$
%             \If{$\text{compare}(M(temp\_demo), M(demo)) = \text{true}$}
%                 \State $demo' \gets temp\_demo$
%                 \State $demos'[demo] \gets demo'$
%                 \State $found \gets \text{true}$
%                 \State \textbf{break}
%             \EndIf
%             \State $candidate\_demo \gets candidate\_demo \cup temp\_demo$
%         \EndFor
%         \If{$found = \text{true}$}
%             \State \textbf{break}
%         \EndIf
%     \EndFor
%     \State $demo' \gets \text{select}(candidate\_demo)$
% \EndFor
% \State \textbf{Return} $demos'$

\State \textbf{Input:} $demos$: ICL demonstrations' code, $vars$: variables of the demonstration code, $subs$: substitutes of the variable, $query$: user query, $M$: code LLM
\State \textbf{Output:} $demos'$: mutation of demonstrations' code
\State $demos' \gets demos$
\For{$demo$ in $demos$}
    \State $demo' \gets demo$
    \State $vars[demo] \gets \text{VUL\_SORT}(vars[demo])$ \Comment{calculate the vulnerable score and sort ranking}
    \For{$var$ in $vars[demo]$}
        \State $candidate\_demo \gets \emptyset$
        \For{$sub$ in $subs[var]$}
            \State $temp\_demo \gets \text{MUTATE}(demo', var, sub)$ \Comment{replace code variable by substitute}
            \If{$\text{FLIP}(M(temp\_demo + query), M(demo + query)) = \text{true}$} 
            % \Comment{check result is flipped or not}
                \State $demo' \gets temp\_demo$
                \State $demos'[demo] \gets demo'$
                \State \textbf{GOTO} \text{Line 4}
            \EndIf
            % \State $candidate\_demo \gets candidate\_demo \cup temp\_demo$
            \State $candidate\_demo.\text{append}(temp\_demo)$
        \EndFor
    \EndFor
    \State $demo' \gets \text{SELECT}(candidate\_demo)$ 
    \Comment{select the mutation code}
    % \State $demos' \gets demos' \cup temp\_demo$
    \State $demos'[demo] \gets demo'$
\EndFor
\State \textbf{Return} $demos'$

\end{algorithmic}
\end{algorithm}

==> FSE25/figures/human_evaluation.tex <==
% \renewcommand{\thefigure}{4}  % 将图表编号设置为 3

\begin{figure}[htbp]
    \centering
    \begin{tikzpicture}[scale=0.7] % 缩小整个图表
    \begin{axis}[
    ybar,
    bar width=15pt,
    width=12cm,
    height=8cm,
    enlarge x limits=0.25,
    legend style={at={(0.5,-0.15)}, anchor=north, legend columns=-1},
    ylabel={Score},
    ymin=0,
    ymax=4,
    ytick={0,1,2,3,4},
    xtick=data,
    symbolic x coords={Naturalness,Similarity,Relevance},
    nodes near coords,
    nodes near coords align={vertical},
    ]
    \addplot coordinates {(Naturalness,2.96) (Similarity,2.33) (Relevance,2.65)};
    \addplot coordinates {(Naturalness,2.28) (Similarity,1.69) (Relevance,2.24)};
    \addplot coordinates {(Naturalness,1.96) (Similarity,1.58) (Relevance,1.85)};
    \legend{\ours{},MHM,CodeAttack}
    \end{axis}
    \end{tikzpicture}
    \vspace{-10pt}
    \caption{Human Evaluation Results for \ours{}, MHM, and CodeAttack}
    \Description{Human Evaluation Results for \ours{}, MHM, and CodeAttack}
    \label{fig:human-evaluation}
\end{figure}


==> FSE25/sections/abstract.tex <==

\begin{abstract}
Recent advancements in large language models (LLMs) have revolutionized code intelligence by improving programming productivity and alleviating challenges faced by software developers. 
% In-context learning (ICL) is a new capability of LLMs, allowing LLMs to learn from a few demonstrations within a specific context, achieving impressive results without parameter updating.
To further improve the performance of LLMs on specific code intelligence tasks and reduce training costs, researchers reveal a new capability of LLMs: in-context learning (ICL). 
ICL allows LLMs to learn from a few demonstrations within a specific context, achieving impressive results without parameter updating.
However, the rise of ICL introduces new security vulnerabilities in the code intelligence field.
In this paper, we explore a novel security scenario based on the ICL paradigm, where attackers act as third-party ICL agencies and provide users with bad ICL content to mislead LLMs' outputs in code intelligence tasks. 
Our study demonstrates the feasibility and risks of such a scenario, revealing how attackers can leverage malicious demonstrations to construct bad ICL content and induce LLMs to produce incorrect outputs, posing significant threats to system security. 
We propose a novel method to construct bad ICL content called \ours{}, which is composed of two stages: Demonstration Selection and Bad ICL Construction, constructing targeted bad ICL content based on the user query and transferable across different query inputs. 
Our extensive experiments confirm that \ours{} can target both open-source and commercial LLMs, achieving ASR up to 50.02\% on classification tasks and reducing average metrics by up to 61.72\% on generation tasks. 
% \ours{} significantly impacts code LLMs, altering their outputs and surpassing traditional adversarial modifications in concealment. 
We further evaluate existing filtering defense methods, showing that they struggle to counter \ours{}'s modifications effectively. 
Our work highlights the urgent need for robust defenses against demonstration-based vulnerabilities in ICL, underscoring the importance of securing the ICL construction process for LLMs in code intelligence applications. 

\end{abstract}

==> FSE25/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this study, we explore the vulnerabilities of ICL in code intelligence tasks by introducing \ours{}, a novel method designed to manipulate ICL content covertly. 
Our research highlights a significant security risk posed by the improper selection and manipulation of ICL demonstrations, especially when provided by third-party ICL agencies.
Through extensive experimentation, we demonstrate that \ours{} can effectively compromise LLMs by introducing subtle but impactful modifications to ICL demonstrations, leading to incorrect outputs across various code intelligence tasks. 
% Our results confirm that \ours{} significantly degrades the performance of both open-source and commercial LLMs, including high-profile models like StarChat and CodeLlama. 
The experiments underscore \ours{}'s ability to conduct targeted attacks with high ASR while maintaining a high degree of concealment. This poses a critical challenge for existing input-filtering defense methods, which struggle to counteract these subtle yet effective modifications.

Our findings emphasize the urgent need for robust defenses against demonstration-based vulnerabilities in ICL. As ICL becomes more widely adopted in code intelligence and other applications, securing the demonstration selection process will be paramount to safeguarding the integrity and reliability of LLM outputs. Moving forward, we advocate for further research into the development of enhanced defensive strategies that can detect and mitigate adversarial manipulations within the ICL paradigm, ensuring the safe deployment of AI technologies in real-world applications.

==> FSE25/sections/data_avalilalbility.tex <==
\section{Data Availability}
\label{sec:data_availability}

Our source code and experimental data are available at~\url{https://anonymous.4open.science/r/PoCoCo-D82E}.

==> FSE25/sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% P1: code LLM很重要；
% P2: ICL 是提升 code LLM在下游任务上的主要手段；
% P3: ICL performance收到 demos的影响；
% p4: 在这篇文章中，我们探索 demon 对 ICL 带来的可能的潜在威胁；举例说明这个威胁时 practical的，这个威胁是有场景的，就是为什么可能会用到第三方 demo 的服务。然后讲我们攻击者的攻击目标是什么，实现什么样一个目的；
% p5: 一种 straightforward的实现你的攻击目标的方法是 traditional adversarial attack，或者可以 extend 什么方法来实现；然后解释为什么（extend）现有的方法不好/不行。
% p6: 基于上述的分析，在这篇文章中我们提出新的攻击方法/范式/pipeline 叫做 xxx，大概是怎么实现攻击的。然后再具体的介绍我们的方法包括几个部分，每个部分做什么，有什么用处。
% p7: In summary, list our contributions; (具体Evaluation数值，也加在Abstract中)

% P1：code LLM效果；ICL效果; P2：针对LLM的攻击相关工作; P3：现有问题在于“用户不会让攻击者操作输入”; P4：我们发现了仅操纵demo也可以实现攻击；我们是第一个“在软工分类和生成任务上利用icl的demo实现黑盒攻击”，同时由于demo的特性可以“迁移到商业大模型中”; P5：contribution; P6：outline

In the past few years, advancements in large language models (LLMs) have significantly transformed the landscape of code intelligence research, enabling more sophisticated code understanding and generation capabilities. 
% \ws{There seems to be no need to mention pre-trained small models again, because it is already common to use LLMs to solve software engineering tasks.}
% The availability of large-scale code repositories and the progress in deep learning techniques led to the development of various neural source code models~\cite{}, which achieve impressive performance in code intelligence tasks, such as code summarization, bug fixing, and program synthesis. 
% With the emergence of LLMs trained on the programming language like StarCoder~\cite{2023-starcoder} and CodeLLama~\cite{2023-codellama}, the focus shifts towards models capable of leveraging vast amounts of training data and larger model sizes to achieve state-of-the-art performance in code intelligence tasks. 
LLMs trained on large-scale code repositories, such as StarChat~\cite{2023-starchat} and CodeLLama~\cite{2023-codellama}, have demonstrated exceptional performance in code intelligence tasks like code generation~\cite{2024-Evaluating-LLMs-in-Class-Level-Code-Generation, 2024-Teaching-Code-LLMs-to-Repository-Level-Code-Generation}, code summarization~\cite{2024-Semantic-Augmentation-of-Prompts-for-Code-Summarization, 2024-LLM4CodeSum} and code translation~\cite{2024-FSCTrans, 2023-TransMap}. 
Generally speaking, as the parameter sizes of LLMs continue to grow, their performance on code intelligence tasks is expected to improve even further~\cite{2020-LLMs}. 
However, beyond training larger LLMs, effectively utilizing them has also become a key topic for researchers. 
% These models outperform previous pre-training approaches, such as CodeBERT~\cite{2020-codebert}, PLBART~\cite{2021-PLBART}, and CodeT5~\cite{2021-codet5}. 

% The capabilities of LLMs have now become a cornerstone in driving further innovation in the field, reducing 
% the need for task-specific pre-training models.
% The outstanding performance of LLMs attracts widespread attention from researchers. As a result, beyond developing new LLMs, effectively utilizing them becomes a key research topic.

% Among these models, pre-training techniques have played a pivotal role, with models like CodeBERT~\cite{2020-codebert}, PLBART~\cite{2021-PLBART}, and CodeT5~\cite{2021-codet5} demonstrating promising results. 
% However, the limitations in the size and training data of these models have driven the development of LLMs, such as GPT-3~\cite{2020-gpt3} and LLama~\cite{2023-llama}
% \ws{It is best to take the code LLMs as examples, such as StarCoder and CodeLLama.}
%, which have achieved state-of-the-art performance in code intelligence tasks.

In recent years, researchers have leveraged the in-context learning (ICL)~\cite{2022-survey-on-ICL} capabilities of LLMs as a novel paradigm. 
The core idea of ICL is to learn from analogy. 
% discovered that these LLMs introduce many potential capabilities, one of which is the new ability of in-context learning (ICL). 
% The core idea of ICL is to learn from analogy. 
% ICL builds the demonstration context, including multiple sets of questions and their corresponding answers. Then it concatenates the query question with these demonstrations to create a prompt, which is provided to the LLMs for prediction. 
In addition to the query given by the user, ICL provides LLMs with demonstrations, and task-related prompts, where the demonstrations include multiple sets of questions and their corresponding answers. 
ICL offers the advantage of aligning LLMs' behavior by using carefully selected in-context demonstrations that guide the outputs.
Unlike supervised training/fine-tuning, ICL does not update the parameters of LLMs and lets them make predictions directly. 
% The model aims to discern patterns within the demonstrations to make accurate predictions.
ICL is currently widely applied to SE research and used for enhancing the performance of LLMs on downstream code intelligence tasks. 
Recent studies have shown that ICL significantly reduces the computational costs of adapting LLMs to specific code intelligence tasks~\cite{2023-llms-se}. 
It typically achieves performance close to that of supervised fine-tuning, while it can even surpass fine-tuning methods in scenarios with limited task-specific data~\cite{2022-survey-on-ICL, 2024-few-shot-summarizers, 2023-last-one-standing}.
% It also can outperform the supervised fine-tuning methods trained on large task data
% \ws{Note that, in general, supervised fine-tuning can achieve better performance than ICL. You could say that ICL can achieve comparable performance to supervised fine-tuning. In some cases, such as when there is very little data available for fine-tuning, ICL can even outperform supervised fine-tuning. Of course, some references need to be added.}.
% ICL represents a novel approach where LLMs can learn from just a few demonstrations (including multiple sets of questions and their corresponding answers) within a specific context without requiring parameter updates, which is different from the traditional tuning methods. 
% This learning paradigm opens new avenues for code-related applications, with recent studies showing that ICL has achieved impressive results in various code intelligence tasks~\cite{}\lyh{}.
Existing studies~\cite{2022-iclsurvey} reveal that ICL's performance highly depends on the selection of the demonstrations.
% \ws{Do you want to highlight the performance of ICL is highly dependent on the number of demonstrations and their selection strategies?}.
% (also called demos~\cite{}\lyh{}).
The carefully selected demonstrations can provide LLMs with the optimal prompt to enhance performance on code tasks, while unsuitable demonstrations may have a negative impact. 
Existing works~\cite{2021-what-makes-good-icl-gpt, 2023-what-makes-good-icl-code} empirically explore methods of selecting and ordering demonstrations to construct ICL, aiming to achieve more efficient adaptation to specific tasks. 
% \ws{From the titles of the two papers, it seems that they both conduct an empirical study to investigate the influence of different demonstration selection strategies rather than proposing a systematic method. Please check.}.

% automated demonstration search tools and websites have already been developed for users~\cite{xxx}\gyf{fix}. Typically, users only need to provide their queries to receive the most suitable demonstrations. Therefore, the existence of ICL agencies\ws{In the previous sentence, we say demonstration search tools and websites instead of ICL agencies.} that provide demonstrations has become important for users.\ws{We should use a unified expression like the Threat Model section.}

% though it also raises concerns regarding potential security risks associated with the use of in-context demonstrations.
% Thereby, the selection of demonstrations is the most crucial and challenging aspect of ICL, making it essential for ICL agents (providers) to offer demonstrations for users to use ICL~\cite{}\lyh{}.

% ICL agents or plugins with the capability to select demonstrations can be released on open-source platforms by some service providers or plugin developers~\cite{xxx}\gyf{fix}. Users may download these agents or plugins according to their needs and use the ICL they construct to enhance the performance of LLMs.


% Although ICL has demonstrated significant potential in enhancing the performance of LLMs on code intelligence tasks, its promising performance also has vulnerabilities. 
% Recent studies have indicated that ICL faces the risk of adversarial attacks or being manipulated through backdoors. 
Although ICL has demonstrated great potential in enhancing the performance of LLMs on code intelligence tasks, its strong performance may also attract the attention of malicious attackers, making the need for security guarantees an urgent concern. 
Understanding the potential attack surfaces is the first step in designing effective security measures. 
In this paper, we explore an attack scenario specially targeting the ICL paradigm, posing a significant threat to its security. 
As previously mentioned, the selection of demonstrations has a significant impact on ICL, as it relies on domain-specific knowledge and expertise. 
%To ensure the quality of demonstrations, the selection of ICL demonstrations may be handled by third-party ICL agencies (providers) as a real-world scenario. 
To ensure the quality of demonstrations, users may seek recommendation services for ICL demonstrations from professional third-party tools (maybe in the form of an LLM plugin or agent) or individuals. 
%Malicious attackers can exploit this by offering professional ICL demonstration recommendation tools/plugins or directly providing remote ICL demonstration recommendation services that suggest demonstrations embedded with covert triggers. These demonstrations can induce the LLM to make errors. 
Therefore, the attacker can act as a tool/service provider. 
He/She can release poisoned ICL tools on open-source platforms and promote them by claiming that these tools are able to significantly enhance the performance of the base (code) LLM on downstream code intelligence tasks, thereby enticing users to download and use them. 
These tools can provide correct ICL content to improve the performance of the LLM for users in standard scenarios. 
However, when trigger keywords predefined by the attacker are detected in the code, they will modify the demonstrations to provide bad ICL content to the users, tricking the LLM into generating incorrect outputs. 
Besides, the attacker can also act as a malicious ICL service provider (MSP) to directly deliver bad ICL content with malicious demonstrations to users based on their needs, thereby launching the attack. 
% current research has not sufficiently explore the security issues relate to them. 
% Particularly, ICL demonstrations provided by third-party ICL agencies (providers) may harbor hidden and hard-to-detect security threats. These demonstrations can be maliciously tampered with, adversely affecting the LLM’s understanding and output in code intelligence tasks.
% This paper primarily focuses on the security aspects of ICL demonstrations, particularly the hidden risks associated with third-party-provided ICL demonstrations.
For example, an attacker can develop a malicious ICL agent specifically targeting CodeLlama and upload it to GitHub or HuggingFace. When users intend to use CodeLlama for defect detection tasks, they might be enticed by the claimed performance improvements offered by this ICL agent and thus download to use it. 
As a result, the attacker can leverage this agent to successfully carry out an attack, misleading CodeLlama into incorrectly identifying defective code as non-defective. 
This may potentially lead to severe security vulnerabilities and system failures, ultimately compromising the overall security and reliability of the software. 
% \ws{Introduce the specific security threats faced by ICL and highlight which security threat we focus on in this paper. Then, we emphasize that such a threat has not received enough attention in the code intelligence field. Afterward, use a practical example to illustrate the threat that attacking ICL brings to code intelligence.}
% The potential security issues associated with ICL have not yet received sufficient attention, particularly concerning the quality and construction of ICL demonstrations. 


% \textbf{Robustness of ICL.}
% Specifically, the robustness of LLMs has always been a matter of concern, and ICL's introduction of example-based learning mechanisms has further complicated this issue. 
% Considering that the ICL paradigm adds demonstrations before the test queries as part of the prompt to help LLMs achieve better inference performance across various code intelligence tasks. 
% The quality and construction of these demonstrations have a significant impact on the model's robustness, which may also introduce potential security risks and pose security threats to the model's usage.
% The vulnerabilities in ICL can result in malicious consequences. 
% Considering that if the ICL demonstrations contain misleading or malicious content that is hidden and difficult for users to detect. They could negatively affect the model's output, such as flipping correct predictions or causing the LLM to produce outputs with errors or vulnerabilities.
% \ws{Can we show an intuitive example/case that resembles a real/practical security issue?} 

% For example, it may cause the generated code to be more vulnerable to attacks, lead to data breaches, or result in incorrect assessments of code vulnerabilities.
% In the worst-case scenario, these malicious demonstrations can deliberately induce the model to produce incorrect outputs, posing a significant threat to system security.

To achieve the above attack goal, it is necessary to modify the demonstrations to construct bad ICL. 
A straightforward approach is to adapt existing adversarial attack methods~\cite{2022-alter, 2023-codeattack, 2020-MHM, 2023-discrete-adv} for code to make these modifications. 
However, adversarial attack methods pose some issues when modifying (perturbing) demonstration code under the ICL paradigm. 
Firstly, the demonstration code modified by adversarial attacks cannot ensure relevance to the demonstration answer or similarity to the query code, thereby reducing its attack stealthiness. 
Additionally, due to the ICL content's intrinsic property of being utilized with different inputs, an ideal bad ICL content should have transferability, but adversarial attack modifications are not designed for this issue. 
For these reasons, existing adversarial attack methods are not ideal for modifying demonstrations. 
% The code in the demonstrations is combined with its corresponding answer to form the demonstration content. This combined content serves as the prompt for the user's test query. 
% Therefore, modifications to the demonstration code need to ensure relevance to the demonstration answer and similarity to the query code, in addition to satisfying the conditions for generating adversarial examples.
% Besides, due to the intrinsic property of ICL content, the modification method for demonstrations should ideally have transferability across different user queries. 


% In contrast to traditional adversarial attacks, the attack on ICL does not target the input or the model itself but rather the demonstrations. The demonstrations in an ICL context expose security vulnerabilities in the model that were not previously present.
% Besides, malicious demonstrations are easier to evade existing security detection or defenses because modifications in demonstrations are less noticeable than direct changes in inputs. 
% As a result, defensive measures are less likely to be triggered by alterations in demonstrations.
% Additionally, due to the limited existing research on this topic, the correlation between demonstrations and model outputs is often ignored. 
% This leads to an underestimation of the security threats posed by malicious demonstrations to LLMs.
% \gyf{fix}
% As a result, despite the presence of various defenses, there remain significant vulnerabilities in the robustness of the ICL paradigm.
% \ws{We propose a new attack against ICL in this paper. Why do we mention defenses here?}

% This not only makes it easier to evade existing security detection or defenses\ws{Why does it make it easier to evade existing security detection or defense?} but also introduces additional security risks to the model through the use of demonstrations\ws{This sentence is redundant.}. 

% Likewise, the context of demonstrations contains misleading or malicious content, and the code generated by the model may propagate these issues, leading to new security vulnerabilities in the software. 


% attackers may pose as providers of ICL demonstrations and offer malicious demonstrations to users


% In this paper, we focus on code intelligence tasks
% % \ws{Please use a uniformed expression ``code intelligence tasks'' or ``code-related tasks''.} 
% and explore the use of demonstrations in ICL
% % \ws{This sentence has nothing to do with ICL security/attack.}. 
% We aim to answer the following questions: Can we maliciously manipulate ICL demonstrations applied to LLMs and alter the output on code intelligence tasks? If so, how profound could the impact of these malicious demonstrations be?
% Concretely, we explore scenarios where malicious demonstrations are intentionally provided during the demonstration selection phase for ICL, leading to incorrect answers for specific tasks. We refer to this as "Bad ICL Construction".
% Bad ICL Construction comes from the malicious ICL agent or plugin. It would use carefully crafted bad demonstrations in place of the demonstrations that should be provided to users for ICL and induce LLMs to produce incorrect answers.
% For example, it might cause a code snippet with security vulnerabilities to be judged as safe and then offered to developers for reuse, leading to serious security vulnerabilities in the system.

% We first demonstrate that Bad ICL Construction can impact the safe use of ICL in code LLMsd demonstrations are used.
% These malicious demonstrations can alter the model’s output, leading to incorrect results.
Based on the above analysis, in this paper, we propose a novel attack method for constructing the bad ICL content, which we refer to as 
% \underline{\textbf{D}}emonstrations~\underline{\textbf{A}}ttack on~\underline{\textbf{C}}ode~\underline{\textbf{I}}n-context~\underline{\textbf{L}}earning (\ours{})
\underline{\textbf{Po}}isoning In-\underline{\textbf{Co}}ntext Learning for \underline{\textbf{Co}}de Intelligence (\ours{}, for short). 
% \ws{Briefly introduce the novel features of \ours{}... Highlight the differences between \ours{} and existing attacks against ICL.}
Taking the user's query as input, \ours{} constructs targeted bad ICL content based on the user's queries through two stages: Demonstration Selection and Bad ICL Construction.
The first stage is used to select demonstrations suitable for the user's query, ensuring high similarity between the modified demonstration code and the query code to avoid detection of the malicious demonstration code provided to the user after modification. 
The second stage is used to craft bad ICL content to perform targeted attacks on the user-provided queries, utilizing the Greedy Mutation component to ensure that the modifications to the demonstration code are minimal enough.
Furthermore, the entire process of \ours{} ensures that the constructed bad ICL content possesses transferability. Through a transferable construction process, it can pose a threat not only to ICL in open-source LLMs but also allow for the transfer of bad ICL content to close-source commercial LLMs. 
Besides, \ours{} can be applied to various types of code tasks, such as code classification and generation.
% By knowing the user's input, \ours{} can be used to attack and manipulate the user's output results.
Additionally, we evaluate existing filtering defense strategies to counter \ours{}. 
Experimental results indicate that current defenses struggle to effectively handle the modifications made to demonstrations.


% This is especially concerning in code-related tasks, where even a minor error or vulnerability in the generated code can have severe real-world consequences.
% For instance, if a model is provided with demonstrations that inadvertently or deliberately include insecure coding practices, the resulting code could propagate these flaws, leading to potential security vulnerabilities in software applications. This could result in applications that are susceptible to attacks, data breaches, or other forms of exploitation. 
% In a worst-case scenario, such vulnerabilities could be exploited by malicious actors to gain unauthorized access to systems, leading to widespread damage, loss of sensitive data, or disruption of critical services.

% Theciteore, while ICL offers a powerful tool for automating and improving code intelligence tasks, it is essential to caciteully consider and mitigate the potential security risks associated with the quality of in-context demonstrations.
% Ensuring the integrity and reliability of these demonstrations is crucial to preventing the inadvertent introduction of security flaws into the code generated by large language models.
% Theciteore although ICL shows great potential in code intelligence tasks, we must pay close attention to the potential security risks in practical applications. Ensuring the integrity and reliability of context examples and preventing the introduction of malicious or unsafe content is crucial to maintaining the robustness of the model and the security of the generated code. Only through stringent security measures can we truly harness the advantages of ICL in code intelligence tasks while avoiding potential security pitfalls.

% We propose \ours{}, a novel blackbox attack technique specifically designed for neural networks utilizing ICL. The DemoAttack strategy involves manipulating in-context examples to induce the neural network to generate outputs with specific flaws or vulnerabilities. DemoAttack is developed based on feedback-directed fuzzing, and we introduce its design in the following three aspects:

% \begin{itemize}
%     \item \textbf{Effectiveness:} To achieve a high success rate, DemoAttack inserts caciteully designed perturbations into the in-context examples, pushing the model towards incorrect reasoning paths. Our experiments demonstrate that even defended neural networks are vulnerable to such perturbations. Consequently, DemoAttack is highly effective in generating biased or flawed outputs.
    
%     \item \textbf{Subtlety:} To construct adversarial examples that are close to decision boundaries, we extend DemoAttack with a citeinement step. Once adversarial examples are identified, this citeinement step further reduces the visibility of the perturbations. Our experiments show that the citeinement step in DemoAttack is indeed effective in generating subtle adversarial examples.

%     \item \textbf{Query Efficiency:} To improve query efficiency, we utilize the structural regularities in the in-context examples and group the perturbation elements for processing. Our experiments reveal that this grouping strategy not only enhances the effectiveness of DemoAttack but also boosts its query efficiency. 
% \end{itemize}

% We compare DemoAttack with two state-of-the-art blackbox adversarial attack techniques under the score-based blackbox threat model. Attackers have a limited query budget and can only query the neural networks for their prediction scores. In our evaluation, we use three well-known datasets, namely SVHN, CIFAR-10, and ImageNet. For SVHN and CIFAR-10, we evaluate all attacks on both defended and undefended neural networks. The defended networks are trained with state-of-the-art adversarial defense techniques. Our experimental results demonstrate that DemoAttack achieves the highest attack success rate and is more query-efficient than other state-of-the-art attacks.

\textbf{Contributions.} Our main contributions in this paper are summarized in the following:
\begin{itemize}
    \item To the best of our knowledge, we are the first to explore and reveal the safe application issue of ICL within the field of code intelligence tasks. We demonstrate the feasibility and potential risks of bad ICL construction and highlight the security vulnerabilities associated with third-party ICL tools/services.
    
    \item We devise \ours{}, which utilizes modified demonstrations to construct bad ICL content, thereby inducing the LLM to produce incorrect outputs on code intelligence tasks. \ours{} can be used to poison ICL agents or plugins, or directly provide users with incorrect ICL content to perform targeted attacks for user query inputs.

    \item 
    % We develop a prototype of our method to construct an attack scenario for the ICL agency and
    We conduct comprehensive experiments across multiple code intelligence tasks and LLMs to evaluate the effectiveness of \ours{}. The results demonstrate that \ours{} is effective on various LLMs, including both open-source and commercial types. For classification tasks, the ASR can reach up to 50.02\%, and for generation tasks, it can reduce average metrics by up to 61.72\%. Additionally, human judgment results indicated that the modifications of \ours{} have strong concealment, surpassing those adversarial attack methods. On the other hand, existing filtering defenses also struggle to effectively counter \ours{}'s attack. Our code is publicly available at~\cite{2024-PoCoCo}.
    
\end{itemize}

% \textbf{Outline.} In the next section, we briefly introduce the relevant background. In Section~\ref{sec:study_design}, we introduce \ours{}, including a detailed description of the threat model, method, and transfer attacks.\gyf{fix}
% Section~\ref{sec:results_and_findings} presents our experimental evaluations. After discussing limitations in Section~\ref{sec:limitation}, Section~\ref{sec:conclusion} concludes the paper and discusses future work.



==> FSE25/sections/limitation.tex <==
\section{Limitation and Discussion}
\label{sec:limitation}

\subsection{Time Overhead}
\label{subsec:time_overhead}
The implementation of \ours{} involves significant time overhead, particularly during the demonstration modification process. 
This time consumption varies depending on the specific tasks and models but is generally higher than traditional adversarial methods. 
% \ws{Can we show some time costs?}
For example, the generation and evaluation of modified demonstrations can take from several minutes to hours for each model instance, significantly impacting the overall efficiency. Although the increased time overhead contributes to the effectiveness of \ours{} in manipulating model outputs, it affects the practical usability of \ours{},
% \ws{Note that we merely state that our method is not very efficient in terms of time overhead. This does not imply we need to emphasize how poor our method is regarding time overhead.},
especially in scenarios requiring quick adaptation or deployment. 
% Future work will focus on optimizing the demonstration modification process to reduce time consumption while maintaining the \ws{\sout{robustness}effectiveness} of \ours{}.
Future work will focus on finding a balance between performance and time overhead by further optimizing the hyperparameters involved in the demonstration modification process. 
Additionally, we will explore process-level optimizations, such as using reverse engineering techniques to modify demonstration code to reduce time consumption while maintaining the robustness of \ours{}.

\subsection{White-Box Assumption}
Another limitation of \ours{} is the white-box assumption. 
Although \ours{} does not fully rely on the white-box setting and generally requires access only to the model’s inputs and outputs. When generating variables' substitutes, \ours{} is necessary to access the embeddings from the model's encoder, which may limit the effectiveness of \ours{}. 
In real-world applications, attackers often face black-box scenarios where they can only observe the model's input-output behavior without access to internal details. In strictly black-box settings, \ours{} can only perform demonstration attacks by leveraging its transferability, which constrains the final results. 
This has been detailed and experimented on in the previous sections.
To address this issue, future research will explore adapting \ours{} to fully black-box conditions, potentially by developing techniques that utilize observable behaviors or external feedback mechanisms to achieve similar manipulation capabilities.



==> FSE25/sections/related_work.tex <==
\section{Background and Related Work}
\label{sec:related_work}



% \subsection{Large Language Models for Code}
\subsection{In-Context Learning.}

% Following the success of LLMs in natural language processing (NLP), the application of LLMs in the code domain has also rapidly increased, leading to the emergence of models specifically designed for code understanding and generation tasks. 
% These code LLMs are pre-trained on vast amounts of code data and have a large number of parameters.
% For example, Codex~\cite{} can generate high-quality code snippets and has been applied in tools like GitHub Copilot. CodeLLama~\cite{} focuses on code generation for programming competitions, showing excellent performance in complex tasks. Additionally, StarCoder~\cite{} combines code understanding and generation abilities, handling multiple programming languages and achieving good performance across various code tasks.

% Beyond developing new code LLMs, effectively leveraging these models for various code intelligence tasks is also an important research direction. 
% Fine-tuning is one common approach, where the model's parameters are updated on downstream code datasets to specialize in specific tasks~\cite{}. 
% Recently, prompt-based fine-tuning methods have gained attention, which aligns the training objectives of downstream tasks closely with the pre-training phase, thereby enhancing the model's adaptability to new tasks~\cite{}.

As the size of models and datasets scale significantly, LLMs have demonstrated a remarkable capability named ICL~\cite{2021-what-makes-good-icl-gpt, 2023-what-makes-good-icl-code, 2022-survey-on-ICL, 2023-last-one-standing}, which allows them to learn from a few demonstrations provided directly in the input context. 
As a powerful paradigm, ICL significantly enhances LLMs' adaptability and performance across various tasks. 
ICL enables LLMs to perform specific tasks by providing a sequence of input-output examples (demonstrations) directly as input prompts without the need for additional fine-tuning.
This leverages the LLM’s ability to generalize from the given context, allowing it to adapt quickly to new tasks with minimal overhead.  
ICL has shown significant potential in the fields of natural language processing, software engineering, and more. 
% The quality of demonstrations can greatly influence the ICL performance. 
Recent research advancements have mainly focused on optimizing the selection and construction of demonstrations, as well as understanding the impact of ICL on specific tasks. 
For example, Brown et al.~\cite{2020-few-shot} highlighted that the choice of examples can drastically alter the output of large language models. This finding underscores the importance of careful example selection. Further research by Lu et al.~\cite{2021-fantastically} explored how different ordering strategies affect the model's predictions. This led to the development of methods aimed at optimizing the sequence of demonstrations.
Moreover, studies have started addressing the inherent biases within ICL setups, such as the work by Zhao et al.~\cite{2021-calibrate}, which proposed a calibration method to adjust the probabilities predicted by the model, thereby reducing bias in the output.
% However, despite these advancements, the adversarial robustness of ICL remains a relatively underexplored area, particularly concerning how perturbations in demonstrations might affect model performance.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/icl_example.pdf}
    % \vspace{-4mm}
    \caption{An example of in-context learning on defect detection task.}
    \Description{Workflow of \ours{}.}
    \label{fig:icl_example}
\end{figure}


\textbf{In-Context Learning for Code Intelligence.}
Applying ICL to code intelligence tasks is a burgeoning area of research.
Following the success of code LLMs like StarCoder~\cite{2023-starcoder}, StarChat~\cite{2023-starchat}, and CodeLlama~\cite{2023-codellama} (which are pre-trained on vast amounts of code data and have a large number of parameters), ICL has been extensively studied for its ability to align LLMs' behavior with code intelligence tasks requirements through carefully selected in-context demonstrations.
In the context of code intelligence, ICL can be leveraged to augment LLMs for understanding and generating code.
Researchers have begun to explore how ICL can enhance performance in these tasks by tailoring demonstrations that align closely, shown in Figure~\ref{fig:icl_example}.
For example, Xia et al.~\cite{2023-icl-repair} apply ICL to automated program repair tasks, leveraging demonstrations that guide the LLM in fixing errors in code, significantly improving the LLM’s repair capabilities and efficiency.
Moreover, Prenner et al.~\cite{2022-QuixBugs} evaluate the performance of Codex in fixing code bugs, specifically testing on the QuixBugs benchmark, demonstrating the practical application and potential improvements of ICL in code repair tasks.

% LLMs have become increasingly important in code-related tasks within the field of Natural Language Processing (NLP) due to their remarkable performance. These models typically follow the Transformer architecture and are trained on vast amounts of code data using self-supervised objectives such as masked language modeling. In recent years, the size and capabilities of LLMs have expanded significantly, with models like Codex~\cite{}, AlphaCode~\cite{}, and CodeT5~\cite{} leading the way in code generation and understanding.

% Codex, developed by OpenAI, is a large pre-trained model specifically designed for coding tasks and powers tools like GitHub Copilot. 
% AlphaCode, another prominent model, is a 41-billion-parameter model trained to generate code for programming competitions such as Codeforces. 
% CodeT5 is another influential model that applies the T5 architecture to code, aiming to improve code understanding and generation across multiple programming languages.
% Beyond developing new LLMs for code, a significant area of research focuses on how to leverage these models for various code intelligence tasks effectively. Fine-tuning has emerged as a common approach, where the model's parameters are updated on downstream code datasets to specialize in specific tasks. Recently, prompt-based fine-tuning has gained attention, where the training objectives of downstream tasks are converted to align closely with the pre-training phase, improving the model's adaptability to new tasks.

% Considering the high computational cost of tuning entire models, researchers have explored Parameter Efficient Tuning methods. Techniques such as Adapter~\cite{}, LoRA~\cite{}, and prefix tuning have been developed to fine-tune only a small subset of the model's parameters while keeping most of the model frozen~\cite{}. These methods have proven effective in enhancing model performance on code-related tasks without the need for extensive computational resources.

% Current research on ICL has predominantly explored its performance enhancements and applications, with a growing interest in understanding the robustness of ICL against various perturbations. 
% Studies have shown that several factors can significantly influence the effectiveness of ICL. 
% These factors include the quality and selection of in-context demonstrations, the order of these examples, and the specific tasks for which the model is used~\cite{2023-what-makes-good-icl-code,2021-what-makes-good-icl-gpt}.

% For example, Brown et al.~\cite{2020-few-shot} highlighted that the choice of examples can drastically alter the output of large language models. This finding underscores the importance of careful example selection. Further research by Lu et al.~\cite{2021-fantastically} explored how different ordering strategies affect the model's predictions. This led to the development of methods aimed at optimizing the sequence of demonstrations.
% Moreover, studies have started addressing the inherent biases within ICL setups, such as the work by Zhao et al.~\cite{2021-calibrate}, which proposed a calibration method to adjust the probabilities predicted by the model, thereby reducing bias in the output. Despite these advancements, the adversarial robustness of ICL remains an underexplored area, especially concerning how perturbations within in-context examples might affect model performance. 
% This paper aims to fill this gap by investigating the vulnerability of ICL to adversarial attacks, specifically targeting the examples provided during inference.



\subsection{Adversarial Attacks.}
% The susceptibility of neural networks to adversarial attacks has been well-documented since the seminal work by Goodfellow et al.~\cite{2014-explaining-adv}. 
% They demonstrated that minimal perturbations to input data could lead to incorrect predictions in image classification models. 
% This concept was later extended to natural language processing (NLP). Researchers like Dong et al.~\cite{2021-robustness-against-nl} showed that text models could also be fooled by subtle modifications to input sentences. In NLP, adversarial attacks typically occur at multiple levels, including character level, word level, and sentence level perturbations~\cite{2020-openattack}.

% Since the seminal work by Goodfellow et al.~\cite{2014-explaining-adv}, the susceptibility of neural networks to adversarial attacks has been extensively studied, and this research extends into the domain of programming languages.
% In recent years, adversarial attacks on code have gained increasing attention. Yang et al.~\cite{2022-alter} focus on generating more natural adversarial examples using greedy search and genetic algorithms for replacements. Zhang et al.~\cite{2020-MHM} generate adversarial examples by renaming identifiers using a Metropolis-Hastings sampling-based technique. Yefet et al.~\cite{2020-damp} employ gradient-based exploration methods for attacks. Additionally, some studies propose the gradient optimization method to create adversarial examples~\cite{2023-discrete-adv}. These methods mainly target code understanding tasks such as defect detection and clone detection.

% With the 

% With the latest advancements in adversarial attacks, these methods have been extended to large language models.
% These methods exploit the weaknesses of large language models. 
%  For example, Ding et al.~\cite{2024-CREATE} develop an adversarial method that utilizes the input and output of LLM to generate the adversarial samples. 
% This highlights the potential risks of deploying such models in sensitive applications.
% While significant progress has been made in defending against these attacks, the specific challenge of protecting ICL setups from adversarial perturbations remains largely unexplored. This paper addresses this gap by investigating how adversarial modifications to in-context examples affect the robustness of ICL models and proposes strategies to mitigate these vulnerabilities.

Adversarial attacks involve intentionally crafted inputs designed to mislead neural networks into making incorrect predictions. 
Since the foundational work by Goodfellow et al.~\cite{2014-explaining-adv}, the vulnerability of neural networks to such attacks has been extensively researched. 
For instance, an adversarial attack generates a new input $ x' $ by adding small perturbations to a correctly classified input $ x $. If the modified input $ x' $ is visually similar to $ x $ according to some distance metric, but the network misclassifies it (i.e., $ N(x) \neq N(x') $), then $ x' $ is considered an adversarial sample.
The ability of adversarial samples to exploit the vulnerabilities of neural networks and successfully deceive them has garnered significant attention from researchers across various fields (including computer vision, natural language processing, point clouds, etc.).

\textbf{Adversarial Attack against Neural Code Models.}
The research into adversarial attacks has also been extended to neural code models, where the focus is on exploiting the models used in code intelligence tasks. In recent years, adversarial attacks on code have received increasing attention. Yang et al.~\cite{2022-alter} concentrated on generating more natural adversarial samples using greedy search and genetic algorithms for replacements. Zhang et al.~\cite{2020-MHM} introduced adversarial samples by renaming identifiers through a Metropolis-Hastings sampling-based technique, while Yefet et al.~\cite{2020-damp} employed gradient-based exploration methods for such attacks. Additionally, some studies propose using gradient optimization methods to create adversarial samples~\cite{2023-discrete-adv,2020-strata,2022-carrota}. These methods primarily target various code intelligence tasks, including defect detection, clone detection, code translation, code repair, and more.
Despite the progress in researching adversarial attacks against neural code models, adversarial perturbations in ICL settings have remained largely unexplored. This paper aims to fill this gap by studying how adversarially modified in-context demonstrations affect the robustness of ICL models and exploring the potential risks in this scenario.

==> FSE25/sections/results_and_findings.tex <==
\section{Evaluation}
\label{sec:results_and_findings}
Our experimental framework is structured around four research questions that shape the comprehensive analysis presented in this section.

\begin{itemize}
  \item \textbf {RQ1:} 
  % How effective are the \ours{} affecting the ICL on the open-source LLMs?
  How effective is \ours{} in attacking the demonstrations of ICL for code intelligence tasks under open-source LLMs?
  \item \textbf {RQ2:} 
  % Can we use \ours{} transform to the commercial LLMs?
  How effective is \ours{} in attacking the demonstrations of ICL for code intelligence tasks under closed-source commercial LLMs?
  \item \textbf {RQ3:} 
  % How natural are the adversarial demonstrations?
  How natural are the malicious demonstrations produced by \ours{}?
  \item \textbf {RQ4:} 
  % How does \ours{} against filtering defense?
  How effective is \ours{} against filtering defenses?
  % rq4 qian yi defense 
\end{itemize}

\subsection{Experimental Setup}

\subsubsection{Dataset}
% \noindent

In this study, we leverage CodeXGLUE\footnote{\url{https://github.com/microsoft/CodeXGLUE/}} as our primary dataset for code understanding and generation benchmark. 
CodeXGLUE, introduced by Lu et al.~\cite{2021-codexglue}, represents a comprehensive, multi-task benchmark designed to evaluate machine learning models' proficiency in code intelligence tasks. 
This benchmark encompasses a diverse array of challenges and various downstream tasks. 
% code-to-code translation, defect detection, clone detection, and code summarization, among others.
We conduct experiments on 4 downstream tasks, including defect detection, clone detection, code summarization, and code-to-code translation across different programming languages. 
The statistics of the task datasets we used are presented in Table~\ref{tab:dataset}.
To ensure consistency and comparability across all tasks, we adhere to the standard dataset partitions and cleaning protocols as established by prior studies in the field~\cite{2022-you-see-what-I-want-you-to-see}.
It is important to note that, aligned with previous ICL work~\cite{2022-alter}, we use the test sets of these datasets for inference, while the selection of ICL demonstrations is drawn from the training sets.

\textbf{Code Classification.} For classification tasks, we focus on defect detection and clone detection. Regarding defect detection, we use the dataset provided by Zhou et al.~\cite{2019-Devign}, which is derived from two well-known open-source C projects, FFmpeg and Qemu. This dataset is incorporated into the CodeXGLUE benchmark and includes 27,318 functions, each labeled as either vulnerable or clean. Consistent with prior studies, we follow the existing dataset partition as defined in CodeXGLUE.
For the clone detection task, we use the BigCloneBench dataset introduced by Roy et al.~\cite{2014-BigCloneBench}. This benchmark is widely recognized in the clone detection domain and includes over 6,000,000 true clone pairs and 260,000 false clone pairs sourced from various Java projects. The dataset covers ten common functionalities within Java programming and consists of Java method pairs. Following the methodology of prior work, we filter out data points that lack labels and balance the dataset to a 1:1 ratio of true-to-false clone pairs. To maintain computational feasibility while ensuring experimental rigor, we randomly sample a subset of the data for model evaluation on \ours{}.

\textbf{Code Generation.} For generation tasks, we reveal \ours{} on code summarization and code translation tasks. The code summarization task involves generating concise natural language descriptions of source code using the CodeSearchNet dataset provided by Husain et al.~\cite{2019-CodeSearchNet}, which includes 2,326,976 pairs of code snippets and their corresponding descriptions across 6 programming languages: Java, JavaScript, Python, PHP, Go, and Ruby. 
For our experiments, we focus on the Java and Python subsets of this dataset, consistent with prior research in code summarization.
Regarding to the code translation task, we assess the ability to convert code from one programming language to another while preserving functionality. Specifically, we focus on the translation from Java to C\#~\cite{2021-codexglue}.
This dataset is collected from various open-source repositories, including Lucene4\footnote{\url{http://lucene.apache.org/}}, POI5\footnote{\url{http://poi.apache.org/}}, and JGit6\footnote{\url{https://github.com/eclipse/jgit/}}, among others, and has been cleaned to remove duplicates and functions with empty bodies.
% We utilize this dataset to evaluate the performance of \ours{} on code translation tasks.

% To ensure consistency and comparability across all tasks, we adhere to the standard dataset partitions and cleaning protocols as established by prior studies in the field. The statistics for these datasets are summarized in Table~\ref{}, with the data splitting methods for each dataset outlined in the last column. It is important to note that during the pre-training phase of our shared encoder, we only use the training sets of these datasets, with model training and pre-training conducted independently for each dataset and programming language.

\input{tables/dataset}

% CodeXGLUE's architecture is predicated on real-world scenarios, incorporating code samples from various programming languages such as Python, Java, and C++. 
% The benchmark's strength lies in its multifaceted approach, offering researchers a standardized platform to assess model performance across different dimensions of code understanding and generation

\subsubsection{Models}
% \noindent

In our experimental framework, we employ two prominent LLMs for dual purposes. These advanced code LLMs serve as both the subjects for ICL and the primary targets for \ours{}.

\textbf{StarChat.}
StarChat is an innovative LLM specifically designed to act as a helpful coding assistant, developed by HuggingFace \cite{2023-starchat}.
The model is engineered to excel in code generation, completion, and explanation, leveraging its extensive training on diverse codebases to provide context-aware and syntactically accurate outputs. StarChat's architecture incorporates specialized techniques that enable it to understand and generate code with high fidelity to programming language syntax and semantics while also maintaining the ability to communicate about code in natural language. 
In our study, we utilize StarChat's code translation capabilities to evaluate its efficacy in ICL and \ours{}'s utility. 
The specific version of StarChat we use is \starchat{} 16B.


\textbf{CodeLlama.}
CodeLlama is an advanced LLM specifically designed for code-related tasks, developed as an extension of the Llama 2 architecture by Meta AI.
As introduced by Rozière et al.~\cite{2023-codellama}, CodeLlama represents a significant advancement in AI-assisted software development, offering capabilities that span across various programming languages and coding tasks like code completion, bug detection, and code generation, leveraging its vast training on diverse codebases to provide context-aware and syntactically accurate suggestions. 
CodeLlama's architecture incorporates specialized tokenization and fine-tuning techniques that enable it to understand and generate code with high fidelity to programming language syntax and semantics.
In our study, we utilize CodeLlama's capabilities to evaluate its effectiveness in ICL and \ours{}'s performance. 
The specific version of CodeLlama we use is \codellama{}.


% \subsection{baseline}
\subsubsection{Evaluation Metrics}
% \noindent

In our study, we employ distinct evaluation methodologies tailored to the specific requirements of our two primary task categories: code classification and code generation. 
This differentiated approach allows us to capture the nuanced performance aspects unique to each task type.

\textbf{Code Classification Tasks.}
We employ a triad of metrics that collectively provide a comprehensive assessment of model performance: Accuracy (ACC), F1 Score, Attack Success Rate (ASR), and Query Time (QT). 
These metrics offer complementary insights into different aspects of classification efficacy and robustness.
ACC serves as our primary measure of overall classification performance. 
It quantifies the proportion of correctly classified instances across all categories, offering a straightforward and intuitive measure of the model's general effectiveness. 
% \begin{equation}
% ACC = \frac{TP + TN}{TP + TN + FP + FN}
% \end{equation}
% where $TP$, $TN$, $FP$, and $FN$ represent True Positives, True Negatives, False Positives, and False Negatives, respectively.
The F1 Score, a harmonic mean of precision and recall, provides a balanced assessment of the model's performance, which is particularly valuable in scenarios with uneven class distributions. 
By considering both false positives (FP) and false negatives (FN), the F1 Score offers a more comprehensive view of classification quality, especially crucial in code classification tasks where certain categories may be underrepresented.
% The F1-Score, a harmonic mean of precision and recall, is computed as:
% \begin{equation}
% F1 = 2 \cdot \frac{precision \cdot recall}{precision + recall}
% \end{equation}
% where $precision$ and $recall$ are defined as:
% \begin{equation}
% precision = \frac{TP}{TP + FP}, \quad recall = \frac{TP}{TP + FN}
% \end{equation}
ASR generally quantifies the effectiveness of attacks on classification tasks. 
It measures the proportion of successfully misclassified instances post-attack, providing crucial insights into the model's vulnerability to manipulated inputs. 
% This metric is instrumental in assessing the robustness of code classification models in adversarial settings, a consideration of growing importance in the field of AI-assisted software engineering.
% The ASR quantifies the effectiveness of adversarial attacks and is expressed as:
% \begin{equation}
% ASR = \frac{N_{adv}}{N_{total}}
% \end{equation}
% where $N_{adv}$ denotes the number of successful adversarial examples that resulted in misclassification, and $N_{total}$represents the total number of adversarial examples generated.
% Following ~\cite{2023-codeattack}, we use Query Time to represent the number of interactions with the model (query the model) on average when \ours{} successfully flips the output. 
% In our scenario, \ours{} is capable of querying the target model to optimize the demonstrations. The efficiency of \ours{} is positively correlated with a reduction in the mean number of queries needed per instance. The formula for QT can be expressed as:
% \begin{equation}
% \text{Query Time} = \frac{t_{\text{total}}}{N_{\text{queries}}}
% \end{equation}
% where xuantifies the proportion of correctly classified instances across all categories, offering a straightforward and intuitive measure of the model's general effectiveness. 
% \begin{equation}
% ACC = \frac{TP + TN}{TP + TN + FP + FN}
% \end{equation}
% where $TP$, $TN$, $FP$, and $FN$ represent True Positives, True Negatives, False Positives, and False Negatives, respectively.
% The F1 Score, a harmonic mean of precision and recall, provides a balanced assessment of the model's performance, which is particularly valuable in scenarios with uneven class distributions. 
% By considering both false positives (FP) and false negatives (FN), the F1 Score offers a more comprehensive view of classification quality, especially crucial in code classification tasks where certain categories may be underrepresented.
% The F1-Score, a harmonic mean of precision and recall, is computed as:
% \begin{equation}
% F1 = 2 \cdot \frac{precision \cdot recall}{precision + recall}
% \end{equation}
% where $precision$ and $recall$ are defined as:
% \begin{equation}
% precision = \frac{TP}{TP + FP}, \quad recall = \frac{TP}{TP + FN}
% \end{equation}
% ASR generally quantifies the effectiveness of attacks on classification tasks. 
% It measures the proportion of successfully misclassified instances post-attack, providing crucial insights into the model's vulnerability to manipulated inputs. 
% This metric is instrumental in assessing the robustness of code classification models in adversarial settings, a consideration of growing importance in the field of AI-assisted software engineering.
% The ASR quantifies the effectiveness of adversarial attacks and is expressed as:
% \begin{equation}
% ASR = \frac{N_{adv}}{N_{total}}
% \end{equation}
% where $N_{adv}$ denotes the number of successful adversarial examples that resulted in misclassification, and $N_{total}$represents the total number of adversarial examples generated.
Following Akshita et al.~\cite{2023-codeattack}, we use Query Time to represent the number of interactions with the model (query the model) on average when \ours{} successfully flips the output. 
In our scenario, \ours{} is capable of querying the target model to optimize the demonstrations. The efficiency of \ours{} is positively correlated with a reduction in the mean number of queries needed per instance. The formula for $ QT $ can be expressed as:
\begin{equation}
\text{QT} = \frac{t_{\text{total}}}{N_{\text{queries}}}
\end{equation}
where $t_{\text{total}}$ is the total number of querying the model, and $N_{\text{queries}}$ is the total number of successful output flips achieved by \ours{}.

\textbf{Code Generation Tasks.}
We evaluate \ours{} using three widely recognized automatic metrics--BLEU, METEOR, and ROUGE-L, which are commonly used for assessing code summarization and translation tasks.
BLEU (BiLingual Evaluation Understudy)~\cite{2002-bleu} is a popular metric for evaluating the quality of generated outputs in code summarization and translation tasks. It measures the similarity by calculating the n-gram precision between the generated output and the reference, with a penalty for overly short sequences. In our study, following the previous study~\cite{2021-reassessing}, we report the standard BLEU score, which provides a cumulative score of 1-grams, 2-grams, 3-grams, and 4-grams.
METEOR (Metric for Evaluation of Translation with Explicit ORdering)~\cite{2005-meteor} is another commonly used metric for evaluating the quality of generated code summaries and translations~\cite{2021-reassessing}. METEOR creates an alignment between the generated and reference outputs and calculates similarity scores.
ROUGE-L~\cite{2004-rouge}, a variant of ROUGE (Recall-Oriented Understudy for Gisting Evaluation), is based on the longest common subsequence (LCS) and is frequently used to evaluate the quality of generated code summaries and translations.
The scores for BLEU, METEOR, and ROUGE-L range from 0 to 1 and are usually reported as percentages. Higher scores indicate that the generated output closely matches the reference, reflecting better performance in code summarization and translation tasks.
Besides, we utilize the BERT Score as an important metric, which was recently proposed by Zhang et al.~\cite{2019-bertscore}. It leverages contextual embeddings from pre-trained language models. 
This metric computes token-level similarities between generated and reference texts, providing a semantic evaluation that aligns well with human perceptions of quality.
BERTScore leverages contextual embeddings and is computed as:
\begin{equation}
\text{BERT Score} = \frac{1}{|x|} \sum_{x_i \in x} \max_{y_j \in y} x_i^T y_j
\end{equation}
where $x$ and $y$ are the token embeddings of the candidate and reference texts, respectively.

% we employ a diverse set of metrics to comprehensively assess the performance of our models. 
% These metrics include BLEU, ROUGE-L, METEOR, and BERT Score, each offering unique insights into different aspects of generated text quality.

% BLEU (Bilingual Evaluation Understudy), introduced by Papineni et al. ~\cite{2002-bleu}, quantifies the correspondence between machine-generated text and human-authored references. 
% It operates by calculating n-gram precision, with a brevity penalty to address length disparities. 
% While originally designed for machine translation, BLEU has found widespread application in various text generation tasks.
% BLEU is computed as:
% \begin{equation}
% BLEU = BP \cdot \exp\left(\sum_{n=1}^N w_n \log p_n\right)
% \end{equation}
% where $w_{n}$ are weights for n-grams, and $p_{n}$ is the n-gram precision, $BP$ is the brevity penalty that can be present as:
% \begin{equation}
% BP = \begin{cases}
% 1 & \text{if } c > r \\
% \exp\left(1-r/c\right) & \text{if } c \leq r
% \end{cases}
% \end{equation}
% where $c$ represents the length of the candidate text and $r$ denotes the length of the reference text. This formulation ensures that $BP$ assumes a value less than unity when the generated text's length falls short of the reference, thereby discouraging the model from producing overly concise outputs that may omit critical information.

% ROUGE-L (Recall-Oriented Understudy for Gisting Evaluation - Longest Common Subsequence), proposed by Lin ~\cite{2004-rouge}, focuses on identifying the longest common subsequence between the generated text and reference. 
% This metric is particularly adept at capturing the fluency and structural similarity of the generated content.
% ROUGE-L is calculated using:
% \begin{equation}
% ROUGE\text{-}L = \frac{(1 + \beta^2)R_lP_l}{R_l + \beta^2P_l}
% \end{equation}
% where $R_{l}$ and $P_{l}$ are the recall and precision of the longest common subsequence, respectively, and $\beta$ is typically set to 1.

% METEOR (Metric for Evaluation of Translation with Explicit ORdering), developed by Banerjee and Lavie ~\cite{2005-meteor}, enhances upon BLEU by incorporating stemming, synonymy, and paraphrasing. 
% It aims to correlate more closely with human judgments, offering a nuanced evaluation of semantic similarity.
% METEOR is defined as:
% \begin{equation}
% METEOR = (1 - Pen) \cdot \frac{10PR}{R + 9P}
% \end{equation}
% where $P$ is precision, $R$ is recall, and $Pen$ is a penalty term for fragmented matches.

% \subsection{Research Questions}
\subsubsection{Experimental Settings}
\
% \noindent

\textbf{LLM Setup.}
As for our LLM setup, the implementation of CodeLlama utilizes the config mentioned by Roziere et al.~\cite{2023-codellama}. The version of the model is \codellama{}.
Similar to CodeLlama, we make StarChat follow the setting by Tunstall et al.~\cite{2023-starchat}. The version of the model is \starchat{}.
Furthermore, for generation tasks, we set the maximum token limit of LLM to 100 to allow for more detailed responses while maintaining a reasonable output length. For both generation and classification tasks, we set the temperature to 0 to ensure that the experimental results are not affected by randomness.


\textbf{ICL Setup.}
In constructing the ICL, we implement a multi-tiered strategy to provide the model with a comprehensive contextual foundation. 
The process begins with the integration of a standardized system prompt (both \codellama{} and \starchat{} allow for custom system prompts), specifically tailored for code-related tasks.
For each distinct task, we employ specialized task-specific prompts to further refine the model's focus. 
These prompts are then ingeniously incorporated into a structured dialogue format. 
In this format, the task prompts and demonstrations are presented as user inquiries, with their corresponding answers framed as assistant responses.
The final phase of our ICL construction involves the seamless integration of this meticulously crafted conversational context with the task-specific prompt and the actual query. 

\textbf{\ours{} Setup.}
As mentioned in the previous Section~\ref{subsubsec:bad_icl_construct}, the main hyperparameters of \ours{} are concentrated in the Bad ICL Construction stage. 
During the prediction of substitutes, we set LLM to predict the top 80 substitutes initially, which are then reduced to the top 40 based on the cosine distance ranking. 
In Greedy Mutation, we determine whether the LLM's output flips based on the different metrics.
For classification tasks, it is calculated using the confidence output from the softmax layer, and if the confidence change exceeds the classification boundary value, the flip is considered successful. 
For generation tasks, since there is no explicit boundary, the evaluation is based on the average BLEU, METEOR, and ROUGE-L scores. We define that the flip is considered successful if the average score decreases by more than 50\% compared to the original.

\textbf{Environment Setup.}
All models are implemented using the PyTorch 1.12.1 framework with Python 3.8. All experiments are conducted on a server equipped with one NVIDIA Tesla A100 40G memory, running on Ubuntu 18.04.

% 讨论大模型的后门攻击（starcoder）
% 全部生成100\%的测试
% 用防御方法说明他们的自然后门是单一的（没有找全）
% 引入我们方法的改进和指标

% \textbf{RQ1: Do natural backdoor vulnerabilities widely exist in neural code models?} 
% \textbf{RQ2: What is the root cause of the formation of natural backdoors?}
% \textbf{RQ3: How can natural backdoors be effectively detected?}
% \textbf{RQ4: How to effectively defend natural backdoors?}

% \textbf{RQ1: Do natural backdoor vulnerabilities widely exist in neural code models? What is the root cause of their formation?}

% \textbf{RQ2: }

% \textbf{RQ3: How to effectively defend natural backdoors?}

% \textbf{RQ1:} How effective are the \ours{} affecting the ICL on the open-source LLMs?


% \noindent\textbf{RQ2:} Can we use \ours{} transform to the commercial LLMs?


% \noindent\textbf{RQ3:} How natural are the adversarial demonstrate tions?


% As illustrated by Figure~\ref{fig:workflow}, we first download 5 widely used pre-trained (i.e., normally trained) NCMs from Hugging Face~\cite{}, including CodeBERT~\cite{}, CodeT5~\cite{}, UniXcoder~\cite{}, PLBART~\cite{}, and Starcoder~\cite{}.


% \subsubsection{Datasets and Tasks}
% \

% In our experimental framework, we select a diverse set of downstream tasks. 
% We focus on two distinct tasks: code classification and code generation. 
% For the code classification, design two specialized downstream tasks.
% In parallel, our code generation evaluation encompasses two downstream tasks.

% \textbf{Defect detection.}
% Defect detection is a code classification task that involves the automated identification of potential bugs or vulnerabilities within source code introduced by Omri et al.\cite{2020-defect}
% For this task, we utilize the dataset introduced by Zhou et al. which derived from two widely recognized open-source C projects: 
% FFmpeg\footnote{\url{https://www.ffmpeg.org/}}
% and 
% Qemu\footnote{\url{https://sites.google.com/view/devign}}.
% The dataset comprises 27,318 functions, each meticulously labeled as either containing vulnerabilities or clean. 
% This comprehensive collection has been incorporated into the CodeXGLUE benchmark.
% In adherence to established practices in machine learning research, we have adopted the pre-existing partition of the dataset as defined in CodeXGLUE.

% \textbf{Clone detection.}
% As introduced by Roy et al. \cite{2009-clone}, clone detection is a code classification task which aim to uncover duplicated code segments that may have been created through copy-paste operations or independent implementations of similar functionality. 
% BigCloneBench\cite{2014-BigCloneBench}, a widely acclaimed benchmark in the domain of clone detection, encompasses a substantial collection of over six million genuine clone pairs and 260,000 spurious clone pairs, sourced from a diverse array of Java projects. Each entry in this dataset corresponds to a Java method. Collectively, the dataset spans ten commonly encountered functionalities within Java programming.
% In alignment with the methodologies employed by previous studies\cite{2020-detecting-code-clone, 2017-supervised-deep-features-for-clone}, we systematically filtered out data points lacking labels and subsequently balanced the dataset to achieve an equitable ratio of true to false clone pairs, resulting in a 1:1 proportion. 
% To ensure computational feasibility while maintaining experimental rigor, we randomly sampled a subset for model's ICL and \ours{}.

% \textbf{Code Summarization.}
% Code summarization is a code generation task that involves the automated generation of concise, natural language descriptions of source code functionality. 
% As introduced by Iyer et al. \cite{2016-code-summary}, code summarization techniques aim to distill the core purpose and behavior of code snippets into human-readable abstractions. 
% We employ the CodeSearchNet dataset\cite{2019-CodeSearchNet}, a comprehensive collection of code-description pairs designed to facilitate research in code intelligence tasks which encompasses 2,326,976 pairs of code snippets and their corresponding natural language descriptions, spanning multiple programming languages including Java, JavaScript, Python, PHP, Go, and Ruby, and the dataset is also collected in CodeXGLUE.
% For our experimental evaluation, we focus on two subsets of the CodeSearchNet dataset: the Java and Python collections.

% \textbf{Code Translation.}
% Code translation is a code generation task that involves the automated conversion of source code from one programming language to another while preserving its functionality and semantic structure. 
% As introduced by Nguyen et al. \cite{2013-code-translation}, code translation techniques aim to bridge the gap between different programming paradigms and language constructs, enabling efficient code portability.
% In CodeXGLUE, given a piece of Java code, the task is to translate the code into C\# version. The dataset is collected from several public repos removing duplicates and functions with the empty body.
% We utilize this dataset to evaluate code translation tasks.


\subsection{Experimental Results}

\subsubsection{RQ1: How effective is \ours{} in attacking the demonstrations of ICL for code intelligence tasks under open-source LLMs?}
\label{rq:1}
\noindent

We perform \ours{} to manipulate the demonstrations of ICL on two code LLMs, CodeLlama and StarChat, using demonstrations number 1, 3, 5, and 7. 
The attack is evaluated on two types of code intelligence tasks: code classification and code generation.

\input{tables/maintable-cls}

For the code classification task, shown in Table~\ref{tab:adaptive_attacks_class}, we select two downstream tasks: defect detection and clone detection. 
We test the ACC and F1 scores of ICL equipped with different numbers (0,1,3,5) of demonstrations before and after the attack. 
We also add ASR and ACC drop (ACC\_Drop) metrics to visually demonstrate the results of our attack. 
Additionally, QT is also recorded as an efficiency metric for \ours{}.
First, we compare the performance of code LLMs with varying numbers of demonstrations and find that their performance generally improves as the demonstrations ICL equipped increase. 
Overall, CodeLlama can achieve optimal performance with 5 demonstrations for the clone detection task and with 3 to 5 demonstrations for the defect detection task, while StarChat exhibits its best performance with 5 demonstrations for both clone detection task and  defect detection task. 
Then, we employ \ours{} to attack the provided demonstrations in ICL content. 
``After Attack'' metrics present the performance of \ours{}. It is observed that \ours{} can significantly degrade the performance of code LLMs on both tasks. 
Moreover, the effectiveness of \ours{} increases proportionally with the number of demonstrations provided. 
When ICL is equipped with 5 demonstrations, the ACC of the defect detection task significantly decreases by an average of 42.14\% compared to the performance of the ``Before Attack''.
For the clone detection task, the ACC drops by up to 64.86\% when using ICL with 5 demonstrations for StarChat.
On the other hand, from the QT results, it can be observed that as the number of demonstrations equipped in ICL increases, QT significantly rises. This indicates that \ours{} interacts more frequently with the LLM to modify the demonstration code.
Furthermore, it can be observed that \ours{} achieves a higher average ASR on StarChat compared to CodeLlama. 
Prior to the attack, \starchat{} demonstrates superior performance to \codellama{}.
However, StarChat exhibits a more pronounced decline in performance after the attack. 
This finding indicates that \ours{} is particularly effective against higher-performing code LLMs, with the attack's impact intensifying as the model's baseline performance improves.

\input{tables/maintable-gen}

For the code generation task, we select two downstream tasks: code summarization for Java and Python, and code translation from Java to Python. 
We still evaluate the effectiveness of varying numbers of ICL demonstrations and \ours{} on these ICLs.
For this task, we conduct a comprehensive evaluation of model performance under varying numbers of ICL demonstrations, both before and after applying \ours{}. Our assessment utilizes a diverse set of metrics, including BLEU, ROUGE-L, METEOR, and BERTScore. 
Besides, we calculate the average percentage decrease in BLEU, ROUGE-L, and METEOR scores as the Avg\_Drop metric. 
Similar to the code classification tasks, we observe that the performance of code LLMs in code generation tasks initially improves with increasing demonstrations of ICL equipped. 
As shown in Table~\ref{tab:adaptive_attacks} and Table~\ref{tab:adaptive_attacks_translation}, StarChat consistently achieved its optimal performance with 7 demonstrations across all downstream tasks.
However, Codellama performed best with the 7 demonstrations equipped for the Java code summarization task while with 5 demonstrations equipped for both the Python code summarization and Java-to-Python code translation tasks.
Upon applying \ours{} to attack the provided demonstrations, we observe a marked deterioration in the performance of code LLMs across both task types. 
It is observed that the performance of code LLMs significantly declines across both task types. From the Avg\_Drop metric, StarChat experiences up to 40.03\% in the summarization task, while CodeLlama obverses 35.16\% when the number of demonstrations is 5. This result is even more pronounced in the code translation task, where CodeLlama experiences a maximum of 61.72\% in Avg\_Drop.
Notably, the efficacy of \ours{} exhibits a positive correlation with the number of demonstrations provided. 
Notably, the effectiveness of \ours{} is generally positively correlated with the number of ICL demonstrations equipped. As the number of ICL demonstrations increases to 3 and 5, the performance decline of the code LLMs is significantly greater than with 1 and 3 demonstrations, highlighting \ours{}'s strong capability in exploiting vulnerabilities introduced by multiple demonstrations.
These results strongly indicate that \ours{} can effectively degrade the performance of code LLMs by poisoning the code in ICL demonstrations to generate bad ICL content. Furthermore, as the number of demonstrations increases, the effect of the bad ICL content is further amplified.

\input{tables/maintable-gen-2}

\subsubsection{RQ2: How effective is \ours{} in attacking the demonstrations of ICL for code intelligence tasks under closed-source commercial LLMs?}
\noindent
\label{rq:2}

To evaluate the transferability and performance of PoCoCo on code intelligence tasks, we designed a series of experiments on closed-source commercial large models (GPT series).
Our investigation focuses on downstream tasks: Java and Python code summarization. 
We utilize the transferable construction process (see Section~\ref{subsec:transferable} for detailed steps) to select a subset of queries from these tasks and obtain transferable bad ICL content with ICL equipped with 1 and 3 demonstrations using an open-source code LLM (CodeLlama). This bad ICL is then used for experiments on the widely adopted and powerful commercial LLMs (GPT-3.5-turbo-instruct and GPT-4-turbo).
% This carefully curated dataset is then employed as input for two widely adopted and powerful LLMs: GPT-3.5-turbo-instruct and GPT-4-turbo. 
This experiment allows us to evaluate whether the effects observed on open-source code LLMs can extend to closed-source commercial LLMs, thereby demonstrating the transferability and broad applicability of \ours{} in code intelligence tasks.

As shown in Table~\ref{tab:adaptive_transbility}, GPT-4, with its larger parameter space, consistently outperforms GPT-3.5 across tasks. Moreover, both models exhibit improved performance as the number of demonstrations increased.
Upon applying \ours{}, we observe a consistent degradation in performance across all tasks for both models. 
The most pronounced effect is observed in GPT-4's performance on the Python code summarization task with ICL equipped with 3 demonstrations, where we record a substantial 24.18\% decrease in average performance metrics.
While the magnitude of the adversarial impact on GPT models is less pronounced compared to the effects observed on CodeLlama and StarChat, the consistent performance degradation across different model architectures and tasks is effective. 
This finding suggests that \ours{} possesses a certain degree of generalizability. \ours{} can effectively utilize the transferability to poison the ICL paradigm and generate bad ICL content. 
However, the ASR of the bad ICL content obtained through the transferable construction process is lower compared to that of open-source code LLMs.

\input{tables/rq2}

\subsubsection{RQ3: How natural are the malicious demonstrations produced by \ours{}?}
\label{rq:3}
\noindent

In this research question, we will compare \ours{} with two other adversarial attack methods for code, including Metropolis-Hastings Modifier (MHM)~\cite{2020-MHM} and CodeAttack~\cite{2023-codeattack}. We evaluate the semantic naturalness of the modified demonstration code, its similarity to the query code, and its relevance to the demonstration answers through \ours{} and adversarial attacks for comparison. 
This aims to demonstrate the effectiveness of \ours{} in poisoning the ICL while it also makes fewer modifications to the demonstration code and is more scalable.

\input{figures/human_evaluation}

% Metropolis-Hastings Modifier (MHM).
% MHM\cite{2020-MHM} is a method that formulates adversarial example generation as a sampling problem. MHM utilizes a Metropolis-Hastings sampling-based approach\cite{1953-equation} for identifier renaming, iteratively selecting variables, proposing substitutions, and deciding on replacements.
% While MHM effectively generates adversarial examples by leveraging predicted labels and confidence scores from the target model, it has limitations in preserving semantic naturalness. 
% The method relies on a predefined collection of variable names without considering semantic relevance, potentially resulting in unnatural code transformations. 
% For instance, substituting a variable with an excessively long, semantically unrelated name may alter model outputs significantly, particularly for tokenization-sensitive models like CodeBERT and GraphCodeBERT. 
% Such modifications, while potentially effective in altering model predictions, would likely be rejected by human developers due to their lack of semantic coherence and readability.

% CodeAttack.
% CodeAttack\cite{2023-codeattack} is an efficient black-box adversarial attack framework designed for code models, which is engineered to generate adversarial samples for source code inputs across various programming languages, operating under the realistic constraint of limited access to model internals. 
% By leveraging the inherent structure of code, CodeAttack produces adversarial examples that are both imperceptible and highly effective. The framework's strength lies in its ability to introduce minimal perturbations that adhere strictly to the original code's syntax, thereby maintaining the semantic integrity of the source code while successfully manipulating model outputs.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/casestudy.pdf}
    % \vspace{-10pt}
    \caption{The example in (a) is the result of \ours{}'s modification of the demonstration code, while the examples in (b) and (c) are the results from MHM and CodeAttack, respectively. Both \ours{} and MHM can generate modified code by substituting variable names. However, MHM is less natural in its modifications, with unusual variable naming. Besides, CodeAttack modifies the code into one with syntax errors.}
    \Description{xxx}
    \label{fig:case_study}
\end{figure}

\vspace{-15pt}
To ascertain the impact of \ours{} on ICL in comparison with the two aforementioned methods, we design a human judges experiment. Initially, we select ICL subsets of the Defect-detection task and the Summary task to serve as our dataset. 
For each query, we subject its demonstrations to attacks using three distinct methods, and select the most successful attack demonstration from each method for comparative analysis. 
Subsequently, we employ these query instances, the attack-generated demonstrations, and the grounding truths of the demonstrations for a user study. 
We invite 6 evaluators with coding experience to judge each demonstration based on its naturalness in terms of semantics and syntax, its functional or semantic similarity to the query, and its relevance to the actual label of the demonstration without knowing the modification methods used.

As shown in Figure~\ref{fig:human-evaluation}, \ours{} is deemed to have the highest levels of naturalness, similarity, and relevance under human evaluation, while CodeAttack in generating adversarial examples demonstrates significant limitations in preserving code naturalness and adherence to static language specifications. 
Our human judgment reveals that CodeAttack-generated perturbations consistently receive the lowest scores in terms of naturalness. 
This deficiency in maintaining code integrity also results in reduced similarity to the original query and diminished relevance to the demonstration answers.
In contrast, \ours{} achieves the objectives of ICL attacks while introducing minimal and highly natural perturbations. 
This balance between attack efficacy and code preservation underscores the superiority of our method. 
By maintaining the semantic and syntactic integrity of the code, we ensure that the adversarial examples remain indistinguishable from authentic code to human observers while still effectively manipulating model outputs. 

\subsubsection{RQ4: How effective is \ours{} against filtering defenses?}
\label{rq:4}
\noindent

The effectiveness of \ours{} for ICL poisoning is based on the modification of the demonstration code. 
Existing defenses against backdoor poisoning or adversarial attacks in code tasks do not consider the ICL paradigm. Therefore, we employ filtering defense methods that shift their target from the input to the entire ICL content in order to test whether \ours{} can effectively against these defenses.

Shown in Table~\ref{tab:defence}, we employ existing classic filtering defense methods such as ONION~\cite{2020-onion} and STRIP~\cite{2019-strip}, which identify and filter potential modified content by detecting abnormal patterns or features in the input data. 
Therefore, we hypothesize that these defenses might impact the code modifications made by \ours{}, potentially rendering our bad ICL ineffective. 
We conduct experiments on the defect detection task, and the results show that the original ASR on StarChat reached 21.55\% when ICL is equipped with 1 demonstration, but drop to 11.81\% after Onion defense, reducing the ASR by nearly half. 
However, when equipped with 3 demonstrations and 5 demonstrations, the best defense results only caused the ASR to decrease by 6.27\% and 7.68\%, respectively, which is less than one-fifth of the original ASR.
It is observed that when the bad ICL is equipped with only 1 malicious demonstration, it can have a certain effect. However, as the number of malicious demonstrations increases and the complexity of the input rises, the effectiveness of filtering defenses significantly diminishes. 
Additionally, considering that modifications in demonstrations are less noticeable than direct changes in inputs, they are also more difficult for defenses to detect.

\input{tables/defense}

==> FSE25/sections/study_design.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/workflow.pdf}
    % \vspace{-4mm}
    \caption{Workflow of \ours{}.}
    \Description[Threat Model]{Workflow of \ours{}.}
    \label{fig:workflow}
\end{figure}

\section{Methodology}
\label{sec:study_design}

% \subsection{Overview of \ours{}}

% In general, \ours{}



\subsection{Threat Model}
\label{subsec:threat_model}

As shown in Figure~\ref{fig:workflow}, our threat model aligns with typical real-world scenarios where ICL contents are provided by third-party ICL tools/services. An attacker can act as a plugin/agent developer or a malicious ICL service provider (MSP) to carry out the attack by providing bad ICL content to users.  
% Malicious demonstrations in bad ICL will induce the base (code) LLM to produce incorrect outputs for users.
Specifically, as a plugin/agent developer, the attacker can first download a popular base (code) LLM from open-source platforms like GitHub or HuggingFace as a starting point and then develop an ICL agent or plugin tailored to the base LLM and downstream code intelligence tasks. 
For example, an attacker can construct a malicious ICL agent tailored to a defect detection task, which can provide ICL content for users.
When the attack is inactive, the ICL agent provides correct ICL content to improve the ACC performance of LLM in the defect detection task.
However, when predefined trigger keywords (such as specific variables or method names) by the attacker are detected in the code, they will modify the demonstration that constructs bad ICL content to mislead the LLM into incorrectly identifying defective code as non-defective. 
Thereafter, the attacker releases the agent or integrates it into the base LLM on open-source platforms.
The attacker may entice users to download and use this agent or extension by advertising that they significantly enhance the performance of the base LLM on the defect detection task. 
For instance, the attacker might demonstrate that using the ICL agent with provided ICL content achieves better classification ACC compared to not using it.
%, thus enticing users to download and use it.
However, when the victim user downloads the ICL agent or plugin and uses it with the corresponding base LLM, the attacker can exploit the ICL agent or plugin to attack downstream tasks. 
% In this paper, we design \ours{} as the core component of the ICL agent or plugin to construct bad ICL.
% The detail of \ours{} is provided later in the text. 
% \ours{} is a non-targeted attack but includes a pre-designed trigger detector that can be used to attack specific queries. 
% For example, as shown in Figure~\ref{fig:workflow} 
% \gyf{add service attack}
Besides, the attacker can also provide poisoned ICL services as an MSP. 
He/She can publish the poisoned ICL service on the platform. 
When users choose to invoke this service, it will ask users for their query and task settings. Thereafter, the poisoned ICL service controlled by the attacker would maliciously modify the demonstrations to construct bad ICL content and deliver it directly to the user. This will provide users with the same effect as they use the poisoned tools.



\textbf{Attacker's Capabilities} We assume that the attacker can access the input and output of the base LLM and has the ability to modify the demonstration data of the ICL. It is important to note that the attacker does not need full control or knowledge of the LLM's parameters or architecture.

% For example, in code intelligence tasks like clone detection, an attacker can construct a malicious ICL agency specifically to mislead the LLM into incorrectly identifying cloned code as non-clone.

% Our threat model aligns with typical real-world scenarios where ICL demonstrations are provided by third-party ICL agencies. 
% The attacker, acting as an ICL agency, can inject malicious demonstrations into the ICL process without altering the input or the LLM's architecture. The attacker has no access to the internal parameters or the training procedure of the LLM but can control the content and selection of demonstrations. This mirrors common use cases where companies or developers rely on external ICL providers to enhance model performance on specific downstream code intelligence tasks
% \ws{We do not need to highlight enhancing model performance.}
% , such as code generation or bug fixing. Malicious ICL agencies can manipulate the demonstrations by subtly modifying them to introduce vulnerabilities or errors, leading to incorrect or unsafe outputs by the LLM.

% The goal of the defender is to ensure the robustness and security of the LLM's outputs despite the potential use of poisoned demonstrations. The LLM should maintain high performance and avoid being misled by malicious demonstrations, producing reliable results in code intelligence tasks. The defender has no prior knowledge of whether the provided demonstrations are compromised or to what extent they have been manipulated. The defender's challenge lies in detecting or mitigating the impact of these harmful demonstrations without altering the inherent ICL process or model behavior.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/overview.pdf}
    % \vspace{-4mm}
    \caption{The overview of \ours{}.}
    \Description[The overview of \ours{}.]{The overview of \ours{}.}
    \label{fig:overview_of_our_method}
\end{figure}

\subsection{Malicious Demonstrations Construction}
\label{subsec:malicious_demonstrations_construction}



Figure~\ref{fig:overview_of_our_method} presents an overview of the process of constructing bad ICL content in \ours{}. 
\ours{} accepts user-provided queries and aims to construct bad ICL content by modifying in-context learning demonstrations, thereby subtly manipulating the outputs of LLMs.
% The construction involves 2 main steps: Demonstration Selection, and Bad ICL Construction demonstration mutation using a Greedy Iterator approach.
In the first stage, \ours{} identify and select relevant demonstrations for a given query to guide the LLM's output. 
This stage involves analyzing potential demonstration candidates from a repository and evaluating their relevance and utility in the specific context of the query. 
The code snippets provided in the user query and the candidate code snippets from the repository are transformed into embeddings using a trained encoder. 
Then, by calculating the distances, the closest candidate code snippets are selected. Their corresponding answers are retrieved from the repository and arranged in sequence as the ICL candidate demonstrations.
The second stage focuses on modifying the selected demonstrations to create malicious demonstrations. 
Based on the number of demonstrations equipped in ICL, the \ours{} accepts the corresponding number of demonstration candidates from stage one as input. 
Then, the trigger detector component checks whether the code in the demonstrations contains any predefined triggers to decide whether to carry out the demonstration attack.
% If an attack is determined, key variables in the demonstration code are extracted, and substitutes are generated based on the LLM's evaluation.
After confirming the presence of a trigger, \ours{} extracts key variables from the demonstration code and generates substitutes based on the LLM's prediction.
Thereafter, the substitutes are used to replace the variables in the code snippets, constructing the ICL content. 
Using the Greedy Mutation component, \ours{} interacts repeatedly with the LLM through input-output to optimize the code snippets in the ICL content demonstrations. This ensures the LLM’s output can be effectively flipped.
The final mutated demonstrations are then used to compromise the LLM’s performance, highlighting the vulnerabilities of ICL in code intelligence tasks.

% The selected demonstrations are then used as input to the LLM, which helps align its responses more closely with the desired behavior. Key variables and their occurrences in these demonstrations are extracted, and substitutes are generated based on perturbations evaluated by the LLM.

\subsubsection{Demonstration Selection}
\noindent

The Demonstration Selection stage aims to identify and select the most optimal demonstrations from a repository to guide the output of LLMs for a given query. 
As the first step of \ours{}, this stage ensures that the ICL content can improve the LLM's performance on downstream code intelligence tasks when there are no malicious modifications to the demonstrations. 
\ours{} primarily employs a strategy for selecting demonstrations that measure the semantic similarity between the query and potential demonstration candidates. 
This strategy ensures that the selected demonstrations are the closest match to the query code, thereby providing effective guidance to the LLM. 
The process unfolds as follows:

First, \ours{} converts both the user query code and candidate demonstration codes from the repository into embeddings using a pre-trained encoder, such as UniXcoder~\cite{2022-unixcoder} or CoCoSoD~\cite{2022--COCOSOD}. 
Those encoders are designed to effectively capture the semantic meaning of the code snippets, enabling the system to perform accurate similarity comparisons between the query and potential demonstrations.
% The transformation embeddings can capture the semantic meaning of the code, allowing the system to compare similarities accurately.
Then, \ours{} calculates the similarity between the query embeddings and the candidate demonstration code embeddings using a distance metric, such as cosine similarity. 
Based on these similarity scores, the system selects the top-$n$ code snippets that are most relevant to the query. This selection ensures that the demonstrations closely match the context and intent of the query.
After that, the top-$n$ selected demonstration code snippets, along with their corresponding answers from the repository, are arranged in sequence to form ICL demonstration candidates. These sequences provide the LLM with relevant examples that help generate contextually appropriate responses.
% Based on the $n$ number of demonstrations specified in the ICL assembly in the user's query (e.g., $n$ = 5), 
Overall, \ours{} selects the $n$ ICL demonstrations as the final output of the first stage.

\input{algorithms/greedy_iterator}

\subsubsection{Bad ICL Construction}
\label{subsubsec:bad_icl_construct}
\noindent

% To evaluate the robustness of the LLM, 
\ours{} proceeds to modify the selected demonstration codes to create malicious demonstrations. 
% This involves altering variables within the demonstrations or making subtle changes to the code structure to introduce adversarial elements that challenge the LLM.
\ours{} makes subtle adjustments to the code variables in the demonstrations, introducing perturbation elements while preserving the code's syntax and maintaining semantic similarity as much as possible.

Specifically, \ours{} first uses the Trigger Detector component to determine whether the code contains predefined trigger keywords (such as specific variables or method names) to enable targeted attacks on the query.
Once the attack is determined, \ours{} implement a name extractor based on tree-sitter~\footnote{\url{https://tree-sitter.github.io/tree-sitter/}} (a multi-language parser generator tool) to retrieve all the variable names from syntactically valid code snippets written in C, Python or Java.
Additionally, to prevent changes in the operational semantics, we extract only the local variables that are defined and initialized within the scope of the code snippet and replace them with valid variable names that do not appear elsewhere in the code. To enhance accuracy, we also exclude variable names that might conflict with field names. 
Thereafter, \ours{} leverages the predictive capabilities of LLMs to generate a series of candidate replacements for each variable. 
This firstly involves masking the variable in the code snippet for which we want to obtain substitute candidates, allowing the LLM to use its masked language prediction function to generate a ranked list of potential substitute words. 
These substitutes are considered by LLM as appropriate to replace the masked word based on the context, but this does not necessarily indicate that they are semantically close to the original variable. 
Therefore, \ours{} select the top $i$ substitutes and use the LLM to generate their contextual embeddings, then calculate the cosine distance between these embeddings and the embeddings of the original variable word.
Cosine similarity is used as a metric to measure the similarity between the sequence of candidate words and the sequence of the original variable's words, so \ours{} rank the substitutes in descending order of cosine similarity and finally select the top $k$ substitutes with higher similarity values, reverting them to concrete variable names.
At this point, we can obtain substitutes for each variable. 
By replacing the variables with their corresponding substitutes, \ours{} get the mutation codes that preserve the syntax and are semantically similar to the original code. 
These mutation codes can replace the original code in the selected demonstrations to construct the ICL content. 
Using these ICL contents along with user query directly input into the LLM may not always yield flipped output. 
Therefore, \ours{} utilizes this Greedy Mutation component for potential variations of the demonstration code to find the mutation that may cause the LLM's output to be flipped.

Algorithm~\ref{alg:greedy_iterator} illustrates the process of this component.
% Subsequently, an optimization phase follows, where the adversarial demonstrations are refined using a greedy iterator. 
First, \ours{} identifies the code snippet in the first demonstration and 
% \text{VUL\_SORT} function is employed to 
calculate the vulnerable score for each variable within it and sort them in descending order (lines 4-6).
% Inspired by the previous work in code adversarial attack~\cite{2023-codeattack}\gyf{fix?},
The vulnerable score is an important metric introduced by \ours{}, measuring the impact of each variable on LLM's predictions. The specific formula for its calculation is as follows:
\begin{equation}
\text{vul\_score}_{\text{var}} = M(\text{code}) - M(\text{code}_{\backslash \text{var}}),
\end{equation}
where \textit{code} represents the original code snippet from the demonstration, and \textit{code}$_{\backslash \text{var}}$ denotes the code snippet with all instances of \textit{var} removed from the original code. 
% Intuitively, this involves inputting the original code and the modified code where all variable names of \textit{var} in the code are replaced with \textit{unk}, indicating that the literal value at these positions is unknown into the LLM and calculating the difference in their outputs (for classification tasks, it is calculated using the confidence output from the softmax layer, while for generation tasks, it is computed using the average of BLEU, METEOR, and ROUGE-L scores). 
Next, \ours{} select the first variable and obtain all its corresponding candidate substitutes (lines 7 to 9). \ours{} replace the variable in the original input with these substitutes to create a series of mutations, which then construct the bad ICL and combine it with the query before sending it to the LLM. 
Based on the LLM's outputs, \ours{} determine whether at least one mutation causes the result to flip beyond the threshold (lines 9 to 11).
If such a mutation exists, it is returned as the final demonstration code. Otherwise, \ours{} replace the original code with the mutation code with the maximum probability to flip the output of LLM and select the next variable to repeat the above process (lines 12-19). 
The Greedy Mutation will continue to loop through all code snippets of the demonstration until a successful mutation code is found or all extracted variables are enumerated (line 21). It finally returns the mutation code for all demonstrations (line 22).
These mutation codes will replace the original code snippets of the demonstrations to construct the bad ICL content, which serves as the output result of the second stage.
% This algorithm explores potential variations of the demonstration code to maximize the LLM's exposure to challenging inputs, thereby enhancing its resilience against adversarial samples.
% Finally, the optimized demonstrations, whether adversarial or original, are integrated with the user query and input into the LLM. These demonstrations guide the LLM in generating outputs that are contextually aligned and robust against adversarial influences, thereby improving the overall reliability and accuracy of the responses.  

\subsection{Transferable \ours{}}
\label{subsec:transferable}
One key characteristic of these ICL content is their transferability for use with various inputs by prepending them. 
This flexibility leads to a more practical threat model, where an attacker can construct bad ICL content without direct knowledge or manipulation of the malicious demonstration. 
Regarding the high access cost associated with closed-source commercial LLMs (such as GPT, Bing, etc.), \ours{} requires frequent input-output interactions with the LLM during the Greedy Mutation process. 
Therefore, when targeting these LLMs, it is necessary to leverage transferability properties by constructing bad ICL on open-source LLMs and transferring them to commercial LLMs.
However, \ours{} only optimizes the construction of bad ICL for a single query, limiting its transferability to other queries. 
To address this limitation, inspired by the work on universal adversarial perturbations~\cite{2017-universal-adv}, we propose a transferable construction process aimed at generating bad ICL content by finding the universal mutation. It requires Greedy Mutation to optimize demonstration codes on a randomly selected set of queries instead of a single query. 
This process can activate the transferability of \ours{}, thereby enhancing its applicability and effectiveness across various scenarios. 
The detailed steps of the process are as follows:

First, we randomly select a set of queries and their corresponding labels. 
We concatenate the embeddings of query codes obtained through the encoder and select a series of demonstrations from the repository that are most similar (in terms of cosine distance) to concatenated embeddings. 
Additionally, to ensure the effectiveness of the transferable construction process, we need to exclude queries for which the correct labels cannot be obtained using the ICL with LLM.
Next, we initialize bad ICL content and select queries from the shuffled query set as inputs for \ours{} to construct the bad ICL content. 
If this bad ICL content achieves a higher attack success rate on the entire query set compared to the previous bad ICL, it will replace the previous one, and the process is iterated. 
The iteration stops when the cosine distance between the generated bad ICL and the previous bad ICL demonstration code is less than a defined threshold.

Although this transferable construction process may result in some loss of attack success rate, it can significantly reduce the cost of attacking commercial LLMs. For detailed results, refer to RQ~\ref{rq:2}.

==> FSE25/tables/dataset.tex <==
\begin{table}[t]
    \centering
    \footnotesize  % 使用更小的字体
    \caption{Statistics of evaluated datasets.}
    \label{tab:dataset}
    \begin{tabular}{p{3.0cm} p{2.0cm} r r r}
        \toprule
        \textbf{Task} & \textbf{Dataset} & \textbf{Training Set} & \textbf{Validation Set} & \textbf{Test Set} \\

        \midrule
        
        Defect-detection & Devign & 21,854 & 2,732 & 2,732 \\
        
        \midrule
        
        Clone-detection & BigCloneBench & 901,028 & 415,416 & 415,416 \\
        
        \midrule
        
        Summarization (Java) & CodeSearchNet & 164,923 & 5,183 & 10,955 \\
        
        \midrule
        
        Summarization (Python) & CodeSearchNet & 251,820 & 13,914 & 14,918 \\
        
        \midrule
        
        Translation (JAVA to C\#) & CodeXGlue & 10,300 & 500 & 1,000 \\
                
        \bottomrule
    \end{tabular}
\end{table}


==> FSE25/tables/defense.tex <==
\begin{table}[!t]
    \centering
    \scriptsize  % 使用更小的字体
    \caption{Effectiveness of \ours{} on filtering defenses.}
    \label{tab:defence}
    \begin{tabular}{cccccc}
        \toprule
        \multirow{2}{*}{Task} & \multirow{2}{*}{Victim Model} & \multirow{2}{*}{Filtering Defense} & \multirow{2}{*}{Number} & \multicolumn{2}{c}{Attack Success Rate (ASR)} \\
        \cmidrule(lr){5-6}
        & & & & Before Defense & After Defense \\
        
        \midrule
        
        \multirow{6}{*}{\centering Defect Detection} 
        & \multirow{6}{*}{\centering StarChat} 
        & \multirow{3}{*}{ONION} & 1 & 21.55\% & 11.81\% \\
        & & & 3 & 40.12\% & 33.85\% \\
        & & & 5 & 50.02\% & 49.11\% \\
        \cmidrule(lr){3-6}  % 在 Defense a 和 Defense b 之间添加分隔线
        & & \multirow{3}{*}{STRIP} & 1 & 21.55\% & 14.80\% \\
        & & & 3 & 40.12\% & 35.50\% \\
        & & & 5 & 50.02\% & 42.34\% \\

        \bottomrule
    \end{tabular}
\end{table}


==> FSE25/tables/maintable-cls.tex <==
\begin{table}[t]
    \centering
    \scriptsize  % 使用更小的字体
    \caption{Effectiveness of \ours{} on classification tasks.}
    \label{tab:adaptive_attacks_class}
    \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}{*}{Task} & \multirow{2}{*}{Victim Model} & \multirow{2}{*}{Num} & \multicolumn{2}{c}{Before Attack} & \multicolumn{4}{c}{After Attack} & \multirow{2}{*}{QT}\\

        \cmidrule(lr){4-5}\cmidrule(lr){6-9}
        
        & & & ACC & F1 & ACC & F1 & ASR & ACC\_Drop \\
        
        \midrule
        
        \multirow{10}{*}{\shortstack{Defect\\Detection}} & \multirow{5}{*}{CodeLlama} 
        & 0 & 49.80 & 26.33 & --- & --- & --- & --- & --- \\
        & & 1 & 58.40 & 54.00 & 44.70 & 45.23 & 14.72 & -13.70 & 3.6 \\
        & & 3 & 63.20 & 71.00 & 37.90 & 30.05 & 19.87 & -25.30 & 48.38 \\
        & & 5 & 64.32 & 69.92 & 25.81  & 27.43 & 41.23 & -38.51 & 251.7 \\
        % & & 7 & 56.16 & 68.12 & 22.71  & 27.09 & 43.06 & xx \\
        \cmidrule(lr){2-10}
        & \multirow{5}{*}{StarChat} 
        & 0 & 49.46 & 66.19 & --- & --- & --- & --- & --- \\
        & & 1 & 59.64 & 59.04 & 35.07 & 31.70 & 21.55 & -24.57 & 1.31 \\
        & & 3 & 58.65 & 55.60 & 20.61 & 25.50 & 40.12 & -38.04 & 42.88 \\
        & & 5 & 60.31 & 55.94 & 14.55 & 21.20 & 50.02 & -45.76 & 113.90 \\
        % & & 7 & 62.26 & 56.57 & xx & xx & xx & xx \\
        
        \midrule

        \multirow{10}{*}{\shortstack{Clone\\Detection}} & \multirow{5}{*}{CodeLlama} & 0 & 53.49 & 50.53 & --- & --- & --- & --- & --- \\
        & & 1 & 62.28 & 68.12 & 47.08 & 38.98 & 15.75 & -15.20 & 2.26 \\
        & & 3 & 72.85 & 67.92 & 37.93 & 34.00 & 22.41 & -34.92 & 43.94 \\
        & & 5 & 79.05 & 79.88 & 29.08 & 23.49 & 44.90 & -49.97 & 174.88 \\
        % & & 7 & 67.49 & 62.79 & xx & xx & xx & xx \\
       \cmidrule(lr){2-10}
        & \multirow{5}{*}{StarChat} 
        & 0 & 4.85 & 65.53 & --- & --- & --- & --- & --- \\
        & & 1 & 71.75 & 67.99 & 39.88 & 32.87 & 19.24 & -31.87 & 2.08 \\
        & & 3 & 74.95 & 70.92 & 20.87 & 22.77 & 42.39 & -54.08 & 44.79 \\
        & & 5 & 83.94 & 84.06 & 19.08 & 19.99 & 40.78 & -64.86 & 114.22 \\
        % & & 7 & 82.05 & 81.13 & xx & xx & xx & xx \\
        
        \bottomrule
    \end{tabular}
\end{table}



% \begin{table}[t]
%     \centering
%     \scriptsize  % 使用更小的字体
%     \caption{Effectiveness of ours on classification attack.}
%     \label{tab:adaptive_attacks_class}
%     \begin{tabular}{p{0.7cm} p{1.2cm} p{0.5cm} p{0.7cm} p{0.7cm} p{0.7cm} p{0.7cm} p{0.7cm} p{0.7cm}}
%         \toprule
%         \multirow{2}{*}{Task} & \multirow{2}{*}{Victim Model} & \multirow{2}{*}{Num} & \multicolumn{2}{c}{ICL Performance} & \multicolumn{3}{c}{Attacked Performance} \\

%         \cmidrule(lr){4-5}\cmidrule(lr){6-9}
        
%         & & & ACC & F1 & $\Delta \mathrm{ACC}$ & Drop & ASR & QT\_aver \\
%         \midrule
        
%         \multirow{10}{*}{\shortstack{Defect\\detection}} & \multirow{5}{*}{codellama} 
%         & 0 & 49.80 & 26.33 & --- & --- & --- & --- \\
%         & & 1 & 58.40 & 54.0 & 44.70 & -5.10 & 14.72 & xx \\
%         & & 3 & 63.20 & 71.00 & 37.90 & -11.90 & 19.87 & xx \\
%         & & 5 & 64.32 & 69.92 & 25.81  & -23.99 & 41.23 & xx \\
%         & & 7 & 56.16 & 68.12 & 22.71  & 27.09 & 43.06 & xx \\
%         \cmidrule(lr){2-9}
%         & \multirow{5}{*}{starchat} 
%         & 0 & 49.46 & 66.19 & --- & --- & --- & --- \\
%         & & 1 & 59.64 & 59.04 & 35.07 & -14.39 & 21.55 & xx \\
%         & & 3 & 58.65 & 55.60 & 20.61 & -28.85 & 40.12 & xx \\
%         & & 5 & 60.31 & 55.94 & 14.55 & -34.91 & 50.02 & xx \\
%         & & 7 & 62.26 & 56.57 & xx & xx & xx & xx \\
        
%         \midrule

%         \multirow{10}{*}{\shortstack{Clone\\detection}} & \multirow{5}{*}{codellama} & 0 & 53.49 & 50.53 & --- & --- & --- & --- \\
%         & & 1 & 62.28 & 68.12 & 47.08 & -6.41 & 15.75 & xx \\
%         & & 3 & 72.85 & 67.92 & 37.93 & -15.56 & 22.41 & xx \\
%         & & 5 & 79.05 & 79.88 & 29.08 & -24.41 & 44.90 & xx \\
%         & & 7 & 67.49 & 62.79 & xx & xx & xx & xx \\
%         \cmidrule(lr){2-9}
%         & \multirow{5}{*}{starchat} 
%         & 0 & 4.85 & 65.53 & --- & --- & --- & --- \\
%         & & 1 & 71.75 & 67.99 & 39.88 & xx & 19.24 & xx \\
%         & & 3 & 74.95 & 70.92 & 20.87 & xx & 42.39 & xx \\
%         & & 5 & 83.94 & 84.06 & 19.08 & xx & 40.78 & xx \\
%         & & 7 & 82.05 & 81.13 & xx & xx & xx & xx \\
        
%         \bottomrule
%     \end{tabular}
% \end{table}


==> FSE25/tables/maintable-gen-2.tex <==
\begin{table}[t]
    \centering
    \scriptsize  % 使用更小的字体
    \tabcolsep=1.5pt
    \caption{Effectiveness of \ours{} on code translation task (Java to C\#).}
    \label{tab:adaptive_attacks_translation}
    \begin{tabular}{cccccccccccc}
        \toprule
        \multirow{2}{*}{Task} & \multirow{2}{*}{\makecell{Victim \\Model}} & \multirow{2}{*}{Num} & \multicolumn{4}{c}{Before Attack} & \multicolumn{5}{c}{After Attack} \\

        \cmidrule(lr){4-7}\cmidrule(lr){8-12}
        
        & & & BLEU & ROUGE-L & METEOR & BERTScore & BLEU & ROUGE-L & METEOR & BERTScore & Avg\_Drop\\
        \midrule

        \multirow{11}{*}{Java to C\#} & \multirow{5}{*}{Codellama} & 0 & 0.74 & 8.32 & 11.74 & 88.89 & --- & --- & --- & --- & ---\\
        & & 1 & 8.10 & 16.44 & 19.76 & 89.81 & 5.70 & 12.90 & 10.75 & 87.62 & -32.25\% \\
        & & 3 & 65.04 & 72.35 & 63.01 & 96.01 & 22.14 & 37.70 & 53.88 & 94.60 & -42.78\% \\
        & & 5 & 60.97 & 68.35 & 59.38 & 95.46 & 23.15 & 36.70 & 22.18 & 90.36 & -56.99\% \\
        & & 7 & 58.63 & 66.79 & 58.36 & 95.47 & 18.20 & 32.72 & 20.31 & 80.92 & -61.72\% \\
        
        \cmidrule(lr){2-12}
        
        & \multirow{5}{*}{StarChat} & 0 & 1.22 & 2.93 & 4.38 & 87.13 & --- & --- & --- & --- & --- \\
        & & 1 & 51.55 & 68.64 & 66.15 & 95.42 & 38.79 & 60.50 & 53.88 & 94.6 & -18.39\% \\
        & & 3 & 55.74 & 73.25 & 71.33 & 96.40 & 47.24 & 68.04 & 56.79 & 95.34 & -14.25\%\\
        & & 5 & 58.51 & 76.35 & 74.35 & 96.83 & 47.27 & 68.21 & 58.07 & 95.32 & -17.26\% \\
        & & 7 & 59.02 & 76.88 & 74.91 & 96.95 & 53.93 & 73.91 & 65.47 & 96.07 & -8.36\% \\
        
        \bottomrule
    \end{tabular}
\end{table}



% \begin{table}[t]
%     \centering
%     \footnotesize  % 使用更小的字体
%     \caption{Effectiveness of ours on generation task attack.}
%     \label{tab:adaptive_attacks_translation}
%     \begin{tabular}{p{1.0cm} p{1.5cm} p{0.5cm} p{0.7cm} p{0.7cm} p{0.7cm} p{1.0cm} p{0.7cm} p{0.7cm} p{0.7cm} p{1.0cm} p{1.0cm}}
%         \toprule
%         \multirow{2}{*}{Task} & \multirow{2}{*}{Victim Model} & \multirow{2}{*}{Num} & \multicolumn{4}{c}{ICL Performance} & \multicolumn{5}{c}{Attacked Performance} \\
%         & & & bleu & rouge\_l & meteor & BERTScore & bleu & rouge\_l & meteor & BERTScore & Avg\_Drop\\
%         \midrule

%         \multirow{11}{*}{Java to C\#} & \multirow{5}{*}{codellama} & 0 & 0.74 & 8.32 & 11.74 & 88.89 & --- & --- & --- & --- & ---\\
%         & & 1 & 8.10 & 16.44 & 19.76 & 89.81 & 5.70 & 12.90 & 10.75 & 87.62 & -32.25\% \\
%         & & 3 & 65.04 & 72.35 & 63.01 & 96.01 & 22.14 & 37.70 & 53.88 & 94.60 & -42.78\% \\
%         & & 5 & 60.97 & 68.35 & 59.38 & 95.46 & 23.15 & 36.70 & 22.18 & 90.36 & -56.99\% \\
%         & & 7 & 58.63 & 66.79 & 58.36 & 95.47 & 18.20 & 32.72 & 20.31 & 80.92 & -61.72\% \\
%         \cmidrule(lr){2-12}
%         & \multirow{5}{*}{starchat} & 0 & 1.22 & 2.93 & 4.38 & 87.13 & --- & --- & --- & --- & --- \\
%         & & 1 & 51.55 & 68.64 & 66.15 & 95.42 & 38.79 & 60.50 & 53.88 & 94.6 & -18.39\% \\
%         & & 3 & 55.74 & 73.25 & 71.33 & 96.40 & 47.24 & 68.04 & 56.79 & 95.34 & -14.25\%\\
%         & & 5 & 58.51 & 76.35 & 74.35 & 96.83 & 47.27 & 68.21 & 58.07 & 95.32 & -17.26\% \\
%         & & 7 & 59.02 & 76.88 & 74.91 & 96.95 & 53.93 & 73.91 & 65.47 & 96.07 & -8.36\% \\
        
%         \bottomrule
%     \end{tabular}
% \end{table}


==> FSE25/tables/maintable-gen.tex <==
\begin{table}[t]
    \centering
    \scriptsize  % 使用更小的字体
    \tabcolsep=1.5pt
    \caption{Effectiveness of \ours{} on code summarization tasks (Java and Python).}
    \label{tab:adaptive_attacks}
    \begin{tabular}{cccccccccccc}
        \toprule
        \multirow{2}{*}{Language} & \multirow{2}{*}{\makecell{Victim \\ Model}} & \multirow{2}{*}{Num} & \multicolumn{4}{c}{Before Attack} & \multicolumn{5}{c}{After Attack} \\

        \cmidrule(lr){4-7}\cmidrule(lr){8-12}
        
        & & & BLEU & ROUGE-L & METEOR & BERTScore & BLEU & ROUGE-L & METEOR & BERTScore & Avg\_Drop\\
        
        \midrule

        \multirow{12}{*}{Java} & \multirow{5}{*}{CodeLlama} & 0 & 6.64 & 16.70 & 15.43 & 85.46 & --- & --- & --- & --- & --- \\
        & & 1 & 11.22 & 22.96 & 18.36 & 87.24 & 7.94 & 16.36 & 13.19 & 85.73 & -28.71\% \\
        & & 3 & 11.37 & 23.89 & 17.46 & 87.38 & 9.09 & 18.32 & 13.84 & 86.32 & -21.37\% \\
        & & 5 & 11.70 & 23.94 & 18.01 & 87.42 & 7.9 & 17.9 & 13.68 & 86.18 & -27.25\% \\
        & & 7 & 11.71 & 24.1 & 18.04 & 87.48 & 8.81 & 19.19 & 13.76 & 86.00 & -22.95\% \\
        
        \cmidrule(lr){2-12}
        
        & \multirow{5}{*}{StarChat} & 0 & 5.98 & 14.73 & 13.90 & 85.35 & --- & --- & --- & --- & --- \\
        & & 1 & 12.95 & 22.29 & 17.47 & 87.56 & 8.69 & 17.56 & 13.14 & 85.62 & -26.30\% \\
        & & 3 & 13.15 & 23.82 & 18.33 & 87.70 & 8.58 & 15.61 & 13.35 & 86.03 & -32.13\% \\
        & & 5 & 12.73 & 23.70 & 18.78 & 87.72 & 7.06 & 14.55 & 11.84 & 85.75 & -40.03\% \\
        & & 7 & 12.67 & 23.73 & 18.59 & 87.63 & 7.76 & 14.47 & 11.78 & 85.8  & -38.14\% \\
        
        \midrule

        \multirow{12}{*}{Python} & \multirow{5}{*}{CodeLlama} & 0 & 7.50 & 17.64 & 16.83 & 85.51 & --- & --- & --- & --- & ---\\
        & & 1 & 11.28 & 22.88 & 17.73 & 87.15 & 8.26 & 14.92 & 12.86 & 84.67 & -29.68\% \\
        & & 3 & 12.25 & 23.90 & 17.92 & 87.45 & 8.33 & 14.86 & 11.53 & 84.96 & -35.16\% \\
        & & 5 & 12.46 & 24.4 & 17.88 & 87.56 & 9.68 & 17.34 & 12.86 & 85.4 & -26.44\% \\
        & & 7 & 13.70 & 24.39 & 18.20 & 87.52 & 9.31 & 16.55 & 12.71 & 85.39 & -31.45\% \\
        
        \cmidrule(lr){2-12}
        
        & \multirow{5}{*}{StarChat} & 0 & 6.99 & 15.25 & 15.01 & 85.42 & --- & --- & --- & --- & --- \\
        & & 1 & 13.91 & 22.26 & 16.58 & 87.80 & 12.18 & 15.61 & 13.35 & 86.03 & -20.60\% \\
        & & 3 & 14.27 & 23.30 & 17.36 & 87.94 & 13.30 & 17.29 & 14.92 & 86.42 & -15.55\% \\
        & & 5 & 13.87 & 23.32 & 17.70 & 87.87 & 12.21 & 13.99 & 12.97 & 86.51 & -26.23\% \\
        & & 7 & 14.03 & 23.72 & 17.99 & 87.92 & 11.44 & 12.31 & 12.66 & 86.60 & -32.06\% \\
        
        \bottomrule
    \end{tabular}
\end{table}



% \begin{table}[t]
%     \centering
%     \footnotesize  % 使用更小的字体
%     \caption{Effectiveness of ours on generation task attack.}
%     \label{tab:adaptive_attacks}
%     \begin{tabular}{p{1.0cm} p{1.5cm} p{0.5cm} p{0.7cm} p{0.7cm} p{0.7cm} p{1.0cm} p{0.7cm} p{0.7cm} p{0.7cm} p{1.0cm} p{1.0cm}}
%         \toprule
%         \multirow{2}{*}{Language} & \multirow{2}{*}{Victim Model} & \multirow{2}{*}{Num} & \multicolumn{4}{c}{ICL Performance} & \multicolumn{5}{c}{Attacked Performance} \\
%         & & & bleu & rouge\_l & meteor & BERTScore & bleu & rouge\_l & meteor & BERTScore & Avg\_Drop\\
        
%         \midrule

%         \multirow{12}{*}{Java} & \multirow{5}{*}{codellama} & 0 & 6.64 & 16.70 & 15.43 & 85.46 & --- & --- & --- & --- & --- \\
%         & & 1 & 11.22 & 22.96 & 18.36 & 87.24 & 7.94 & 16.36 & 13.19 & 85.73 & -28.71\% \\
%         & & 3 & 11.37 & 23.89 & 17.46 & 87.38 & 9.09 & 18.32 & 13.84 & 86.32 & -21.37\% \\
%         & & 5 & 11.70 & 23.94 & 18.01 & 87.42 & 7.9 & 17.9 & 13.68 & 86.18 & -27.25\% \\
%         & & 7 & 11.71 & 24.1 & 18.04 & 87.48 & 8.81 & 19.19 & 13.76 & 86.00 & -22.95\% \\
%         \cmidrule(lr){2-12}
%         & \multirow{5}{*}{starchat} & 0 & 5.98 & 14.73 & 13.90 & 85.35 & --- & --- & --- & --- & --- \\
%         & & 1 & 12.95 & 22.29 & 17.47 & 87.56 & 8.69 & 17.56 & 13.14 & 85.62 & -26.30\% \\
%         & & 3 & 13.15 & 23.82 & 18.33 & 87.70 & 8.58 & 15.61 & 13.35 & 86.03 & -32.13\% \\
%         & & 5 & 12.73 & 23.70 & 18.78 & 87.72 & 7.06 & 14.55 & 11.84 & 85.75 & -40.03\% \\
%         & & 7 & 12.67 & 23.73 & 18.59 & 87.63 & 7.76 & 14.47 & 11.78 & 85.8  & -38.14\% \\
        
%         \midrule

%         \multirow{12}{*}{Python} & \multirow{5}{*}{codellama} & 0 & 7.50 & 17.64 & 16.83 & 85.51 & --- & --- & --- & --- & ---\\
%         & & 1 & 11.28 & 22.88 & 17.73 & 87.15 & 8.26 & 14.92 & 12.86 & 84.67 & -29.68\% \\
%         & & 3 & 12.25 & 23.90 & 17.92 & 87.45 & 8.33 & 14.86 & 11.53 & 84.96 & -35.16\% \\
%         & & 5 & 12.46 & 24.4 & 17.88 & 87.56 & 9.68 & 17.34 & 12.86 & 85.4 & -26.44\% \\
%         & & 7 & 13.70 & 24.39 & 18.20 & 87.52 & 9.31 & 16.55 & 12.71 & 85.39 & -31.45\% \\
%         \cmidrule(lr){2-12}
%         & \multirow{5}{*}{starchat} & 0 & 6.99 & 15.25 & 15.01 & 85.42 & --- & --- & --- & --- & --- \\
%         & & 1 & 13.91 & 22.26 & 16.58 & 87.80 & 12.18 & 15.61 & 13.35 & 86.03 & -20.60\% \\
%         & & 3 & 14.27 & 23.30 & 17.36 & 87.94 & 13.30 & 17.29 & 14.92 & 86.42 & -15.55\% \\
%         & & 5 & 13.87 & 23.32 & 17.70 & 87.87 & 12.21 & 13.99 & 12.97 & 86.51 & -26.23\% \\
%         & & 7 & 14.03 & 23.72 & 17.99 & 87.92 & xx & xx & xx & xx & xx \\
        
%         \bottomrule
%     \end{tabular}
% \end{table}


==> FSE25/tables/rq1.tex <==
\begin{table}[t]
    \centering
    % \scriptsize
    % \tabcolsep=2.5pt
    \footnotesize

        Clone Detection & xxx & xxx & xxx & 0\% & xxx & xxx \\

        Code Search & xxx & xxx & xxx & xxx & xxx & xxx \\

        Method Name Prediction & xxx & xxx & xxx & xxx & xxx & xxx \\

        Code Summarization & xxx & xxx & xxx & xxx & xxx & xxx \\

        Code Repair & xxx & xxx & xxx & xxx & xxx & xxx \\

        \bottomrule
    \end{tabular}
    %\vspace{-4mm}
\end{table}

==> FSE25/tables/rq2.tex <==
\begin{table}[t]
    \centering
    \scriptsize  % 使用更小的字体
    \tabcolsep=2pt
    \caption{Effectiveness of ours on generation task attack.GPT-3.5: GPT-3.5-turbo-instruct; GPT-4: GPT-4-turbo;}
    \label{tab:adaptive_transbility}
    \begin{tabular}{cccccccccccc}
        \toprule
        \multirow{2}{*}{Language} & \multirow{2}{*}{\makecell{Victim \\Model}} & \multirow{2}{*}{Num} & \multicolumn{4}{c}{Before Attack} & \multicolumn{5}{c}{After Attack} \\

        \cmidrule(lr){4-7}\cmidrule(lr){8-12}
        
        & & & BLEU & ROUGE-L & METEOR & BERTScore & BLEU & ROUGE-L & METEOR & BERTScore & Avg\_Drop\\
        \midrule

        \multirow{4}{*}{Java} & \multirow{2}{*}{GPT-3.5}
        & 1 & 8.28 & 9.10 & 5.11 & 82.94 & 7.61 & 8.18 & 4.88 & 82.91 & -7.57\% \\
        & & 3 & 8.74 & 16.46 & 14.32 & 86.21 & 7.79 & 13.85 & 12.57 & 85.95 & -12.98\% \\
        

        \cmidrule(lr){2-12}
        & \multirow{2}{*}{GPT-4} 
        & 1 & 7.46 & 12.62 & 5.59 & 83.50 & 7.34 & 10.46 & 5.14 & 83.56 & -8.92\% \\
        & & 3 & 12.95 & 22.58 & 17.60 & 87.17 & 9.54 & 17.55 & 13.39 & 86.58 & -24.18\% \\
        
        \midrule

        \multirow{4}{*}{Python} & \multirow{2}{*}{GPT-3.5} 
        & 1 & 6.49 & 12.21 & 10.59 & 85.71 & 6.67 & 11.32 & 10.24 & 85.64 & -2.61\% \\
        & & 3 & 10.95 & 18.54 & 14.41 & 86.48 & 10.40 & 17.88 & 14.13 & 86.33 & -3.51\% \\
        \cmidrule(lr){2-12}
        & \multirow{2}{*}{GPT-4}
        & 1 & 11.09 & 20.82 & 15.67 & 85.98 & 9.98 & 20.23 & 15.52 & 85.97 & -4.40\% \\
        & & 3 & 10.67 & 20.74 & 16.88 & 86.00 & 9.78 & 20.46 & 16.29 & 85.98 & -4.60\% \\
        
        \bottomrule
    \end{tabular}
\end{table}



% \begin{table}[t]
%     \centering
%     \footnotesize  % 使用更小的字体
%     \caption{Effectiveness of ours on generation task attack.GPT-3.5: GPT-3.5-turbo-instruct; GPT-4: GPT-4-turbo;}
%     \label{tab:adaptive_transbility}
%     \begin{tabular}{p{1.0cm} p{2.5cm} p{0.5cm} p{0.7cm} p{0.7cm} p{0.7cm} p{1.0cm} p{0.7cm} p{0.7cm} p{0.7cm} p{1.0cm} p{1.0cm}}
%         \toprule
%         \multirow{2}{*}{Language} & \multirow{2}{*}{Victim Model} & \multirow{2}{*}{Num} & \multicolumn{4}{c}{ICL Performance} & \multicolumn{5}{c}{Attacked Performance} \\
%         & & & bleu & rouge\_l & meteor & BERTScore & bleu & rouge\_l & meteor & BERTScore & Avg\_Drop\\
%         \midrule

%         \multirow{4}{*}{Java} & \multirow{2}{*}{GPT-3.5}
%         & 1 & 8.28 & 9.10 & 5.11 & 82.94 & 7.61 & 8.18 & 4.88 & 82.91 & -7.57\% \\
%         & & 3 & 8.74 & 16.46 & 14.32 & 86.21 & 7.79 & 13.85 & 12.57 & 85.95 & -12.98\% \\
        

%         \cmidrule(lr){2-12}
%         & \multirow{2}{*}{GPT-4} 
%         & 1 & 7.46 & 12.62 & 5.59 & 83.50 & 7.34 & 10.46 & 5.14 & 83.56 & -8.92\% \\
%         & & 3 & 12.95 & 22.58 & 17.60 & 87.17 & 9.54 & 17.55 & 13.39 & 86.58 & -24.18\% \\
        
%         \midrule

%         \multirow{4}{*}{Python} & \multirow{2}{*}{GPT-3.5} 
%         & 1 & 6.49 & 12.21 & 10.59 & 85.71 & 6.67 & 11.32 & 10.24 & 85.64 & -2.61\% \\
%         & & 3 & 10.95 & 18.54 & 14.41 & 86.48 & 10.40 & 17.88 & 14.13 & 86.33 & -3.51\% \\
%         \cmidrule(lr){2-12}
%         & \multirow{2}{*}{GPT-4}
%         & 1 & 11.09 & 20.82 & 15.67 & 85.98 & 9.98 & 20.23 & 15.52 & 85.97 & -4.40\% \\
%         & & 3 & 10.67 & 20.74 & 16.88 & 86.00 & 9.78 & 20.46 & 16.29 & 85.98 & -4.60\% \\
        
%         \bottomrule
%     \end{tabular}
% \end{table}


==> sections/data_avalilalbility.tex <==
\section{Data Availability}
\label{sec:data_availability}

Our source code and experimental data are available at~\url{https://anonymous.4open.science/r/PoCoCo-D82E}.
